Multi-wavelength Photometric Study of RR Lyrae Variables in the Globular Cluster NGC 5272 (Messier 3)

We present a comprehensive photometric study of RR Lyrae stars in the M3 globular cluster, utilising a vast dataset of 3140 optical ($UBVRI$) CCD images spanning 35 years from astronomical data archives. We have successfully identified previously known 238 RR Lyrae stars from the photometric data, comprising 178 RRab, 49 RRc, and 11 RRd stars. Multi-band periodogram was used to significantly improve the long-term periods of $65\%$ of RR Lyrae stars in our sample, thanks to the unprecedentedly long temporal coverage of the observations. The light curve templates were used to obtain accurate and precise mean magnitudes and amplitudes of all RR Lyrae variables. We combined optical ($UBVRI$) and near-infrared (NIR, $JHK_{s}$) photometry of RR Lyrae variables to investigate their location in the colour-magnitude diagrams as well as the pulsation properties such as period distributions, Bailey diagrams and amplitude ratios. The Period-Luminosity relations in $R$ and $I$ bands and Period-Wesenheit relations were derived after excluding outliers identified in CMDs. The Period-Wesenheit relations calibrated via the theoretically predicted relations were used to determine a distance modulus of $\mu = 15.04 \pm 0.04 \,{\rm (stats)} \pm 0.19 \,{\rm {(syst.)}}$ mag (using metal-independent $W_{BV}$ Wesenheit) and $\mu = 15.03 \pm 0.04 \,{\rm (stats)} \pm 0.17 \,{\rm {(syst.)}}$ mag (using metal-dependent $W_{VI}$ Wesenheit). Our distance measurements are in excellent agreement with published distances to M3 in the literature. We also employed an artificial neural network based comparison of theoretical and observed light curves to determine physical parameters (mass, luminosity, and effective temperature) for $79$ non-Blazhko RRab stars that agree with limited literature measurements.

==> tables/NGC5272_1.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{rlllllllllr}
\hline
No. & Run Name & Dates & Telescope & Camera & U & B & V & R & I & Multiplex \\ 
\hline
   1 &     cf84 &        1984 Jun 22 & Maunakea CFHT 3.6m &        RCA1 & --- &   1 &   1 & --- & --- &       --- \\
   2 &     kp36 &        1985 Jun 12 &          KPNO 0.9m &         RCA & --- &   4 &   4 & --- & --- &       --- \\
   3 &     kp4m &     1985 Jun 16-18 &            KPNO 4m &         RCA & --- &   6 &   5 & --- & --- &       --- \\
   4 &     cf85 &     1985 Jun 20-24 & Maunakea CFHT 3.6m &        RCA1 & --- &  10 &  10 & --- & --- &       --- \\
   5 &      jvw & 1986 Mar 29-Apr 09 &  La Palma INT 2.5m &         RCA &   4 &   6 &   8 &   9 &   6 &       --- \\
   6 &       km &        1986 May 08 &  La Palma INT 2.5m &         RCA & --- &   1 &   2 & --- & --- &       --- \\
   7 &  c91ic41 &        1991 Apr 08 & Maunakea CFHT 3.6m &       lick1 & --- &   2 &   2 & --- &   2 &       --- \\
   8 &     cf91 &     1991 Jul 06-07 & Maunakea CFHT 3.6m &       Lick2 & --- &   2 &   2 & --- & --- &       --- \\
   9 &     saic &        1992 May 25 & Maunakea CFHT 3.6m & HRCam/saic1 & --- & --- &  16 &  15 & --- &       --- \\
  10 &   h92ic1 &        1992 May 27 & Maunakea CFHT 3.6m &       HRCam & --- &   7 & --- & --- & --- &       --- \\
  11 &     cf92 &     1992 Jun 08-09 & Maunakea CFHT 3.6m &        RCA4 & --- &   3 & --- & --- & --- &       --- \\
  12 &    bolte &     1994 Apr 13-16 &          KPNO 2.1m &        t1ka & --- & --- &  30 & --- &  31 &       --- \\
  13 &     cf94 &        1994 Jun 06 & Maunakea CFHT 3.6m &      Loral3 & --- &   4 & --- & --- &   4 &       --- \\
  14 &      jka &        1995 Mar 27 &  La Palma INT 2.5m &        TEK3 & --- &   3 &   8 & --- & --- &       --- \\
  15 &    bond9 &     1997 May 08-10 &          KPNO 0.9m &        t2ka & --- &   4 &   4 & --- &   4 &       --- \\
  16 &      arg &        1997 May 31 &    La Palma JKT 1m &        TEK2 & --- & --- &   3 & --- &   6 &       --- \\
  17 &   bond11 &     1998 Mar 21-22 &          KPNO 0.9m &        t2ka & --- &   9 &   9 & --- &   9 &       --- \\
  18 &  int9804 &        1998 Apr 12 &  La Palma INT 2.5m &         WFC & --- &   3 & --- &   4 & --- &       --- \\
  19 &      dmd &        1998 Jun 24 &    La Palma JKT 1m &        TEK4 & --- & --- &   2 & --- &   2 &       --- \\
  20 &     tng2 &        2000 Feb 04 &  La Palma TNG 3.6m &         OIG &   2 &   2 &   2 & --- & --- &      x  2 \\
  21 &  int0005 &     2000 May 24-28 &  La Palma INT 2.5m &         WFC & --- &   3 &   3 & --- & --- &      x  4 \\
  22 &    jun00 &        2000 Jun 04 & Maunakea CFHT 3.6m &      CFH12K & --- & --- &   2 & --- & --- &      x 12 \\
  23 &   cf0102 &     2001 Feb 16-17 & Maunakea CFHT 3.6m &      CFH12K & --- &  15 &  18 & --- &  12 &      x 12 \\
  24 &   not017 &     2001 Jul 11-15 &  La Palma NOT 2.6m &        CCD7 & --- &   9 &   7 & --- &  10 &       --- \\
  25 &  int0202 &     2002 Feb 03-04 &  La Palma INT 2.5m &         WFC & --- & 112 & 113 & --- & --- &      x  4 \\
  26 &   hannah &        2002 Mar 29 &    La Palma JKT 1m &        SIT2 & --- &   5 &  11 &  10 & --- &       --- \\
  27 &  int1005 &     2010 May 25-30 &  La Palma INT 2.5m &         WFC & --- &  32 &  33 &  33 &  11 &      x  4 \\
  28 &  int1202 &     2012 Feb 22-23 &  La Palma INT 2.5m &         WFC &  16 & --- & --- & --- & --- &      x  4 \\
  29 &  int1204 &     2012 Apr 23-26 &  La Palma INT 2.5m &         WFC &  10 &   9 &   9 & --- &   6 &      x  4 \\
  30 &  int1304 &        2013 Apr 13 &  La Palma INT 2.5m &         WFC &  10 & --- & --- & --- & --- &      x  4 \\
  31 & spm1405a &        2014 May 21 & S Pedro Martir 0.8 &    E2V-4290 &   1 &   2 &   2 &   2 &   2 &       --- \\
  32 &     dahl &     2014 Jun 19-25 & Maria Mitchell 0.4 & Roper PVCAM & --- & --- &   3 &   3 & --- &       --- \\
  33 &  int1501 &        2015 Jan 30 &  La Palma INT 2.5m &         WFC & --- &   2 &   2 & --- & --- &      x  4 \\
  34 &  int1502 &     2015 Feb 25-27 &  La Palma INT 2.5m &         WFC & --- &   9 &   9 & --- & --- &      x  4 \\
  35 &  int1504 &     2015 Apr 24-27 &  La Palma INT 2.5m &         WFC & --- &  16 &  17 & --- &   8 &      x  4 \\
  36 &  int1605 & 2016 May 28-Jun 02 &  La Palma INT 2.5m &         WFC &   1 &  11 &  11 & --- &  10 &      x  4 \\
  37 &  int1704 &     2017 Apr 03-05 &  La Palma INT 2.5m &         WFC & --- &   6 &   6 & --- &   6 &      x  4 \\
  38 &   iac80a &     2017 Jun 17-19 &   Teide IAC80 0.8m &     CAMELOT &   2 &   2 &   2 &   2 &   2 &       --- \\
  39 & spm1801b &        2018 Jan 28 & S Pedro Martir 0.8 &    E2V-4240 &   2 &   2 &   2 &   2 &   2 &       --- \\
  40 &  int1802 &        2018 Feb 22 &  La Palma INT 2.5m &         WFC &   3 &   3 & --- & --- & --- &      x  4 \\
  41 &  spm1802 &        2018 Feb 26 & S Pedro Martir 2.1 &    E2V-4240 &   3 &   3 &   2 &   3 &   3 &       --- \\
  42 &  int1805 &     2018 May 20-22 &  La Palma INT 2.5m &         WFC &   6 &   2 &   6 &   2 & --- &      x  4 \\
  43 &  int1806 &        2018 Jun 12 &  La Palma INT 2.5m &         WFC &   2 &   2 & --- &   2 & --- &      x  4 \\
  44 &  int1906 &     2019 Jun 26-29 &  La Palma INT 2.5m &         WFC &   5 &   2 & --- & --- & --- &      x  4 \\
  \hline
\end{tabular}
}

\begin{minipage}{\textwidth}
\vspace{0.1cm}
\small \textbf{Notes}. 1. Observers R. D. McClure and D. A. VandenBerg 2. Observer P. B. Stetson 3. Observer P. B. Stetson 4. Observers J. E. Hesser and D. A. VandenBerg 5. Observer "JVW" 6. Observer "KM" 7. Observers H. Richer and G. Fahlman 8. Observers P. B. Stetson and J. E. Hesser 9. Observers Bolte and Hesser 10. Observers Richer and Buonanno 11. Observers P. B. Stetson and M. Bolte 12. Observer M. Bolte 13. Run ID 94IC15, observers D. A. VandenBerg and P. B. Stetson 14. Observer "JKA" 15. Proposal KP2771, observer H. E. Bond; includes observations in Sloan u filter 16. Observer A. Rosenberg 17. Proposal 98A-0351, observer H. E. Bond 18. Details unavailable 19. Run number 4064, observer "DMD" 20. Observers Ortolani, Bragaglia and "admin" 21. Proposal P14, observer Robert Greimel 22. Run ID 00AC14, observers Stetson and Fahlman 23. Run IDs 01AK1 and 01AF43, observers Park, Sohn and Oh;  R. Ibata and C. Pichon 24. Observer Bruntt 25. Proposal P20, observer G. Gilmore 26. Proposal "ING\_Science," observer Javier Mendez 27. Proposal N5, observer vdWerf 28. Proposal C34, observer Carrera 29. Proposal c70, observer Milone 30. Proposal C143, observer M. Monelli 31. Observers Ricci et al. and Ayala-Michel; data contributed by Raul Michel Murillo 32. Observer E. Dahl 33. Proposals CAT\_S and N22W, observers Oscoz and Vats 34. Proposal C115, observer C. Martinez 35. Proposal N2, observer Henk Hoekstra; proposal C115, observer Clara Martinez 36. Proposal C143, observer Monelli 37. Proposals "(16A)C143" and "CAT\_S," observer M. Monelli 38. Observer M. Monelli 39. Observers Omar and Raul; data contributed by Raul Michel Murillo 40. Proposal C14, observer M. Monelli 41. Observers "ing" and Michel; data contributed by Raul Michel Murillo 42. Proposal C14, observer M. Monelli 43. Proposal C14, observers Monelli and Rusakov 44. Proposal C143, observer Monelli.
\end{minipage}

==> tables/table_1.tex <==
% \usepackage{graphicx}

\resizebox{\textwidth}{!}{
\begin{tabular}{rlllllllllll} 
\hline
No. & Run Name & Dates & Telescope & Camera & U & B & V & R & I & Other & Multiplex \\ 
\hline
1 & cf84 & 1984 Jun 22 & Maunakea CFHT 3.6m & RCA1 & — & 1 & 1 & — & — & — &  \\
2 & kp36 & 1985 Jun 12 & KPNO 0.9m & RCA & — & 4 & 4 & — & — & — &  \\
3 & kp4m & 1985 Jun 16-18 & KPNO 4m & RCA & — & 6 & 5 & — & — & — &  \\
4 & cf85 & 1985 Jun 20-24 & Maunakea CFHT 3.6m & RCA1 & — & 10 & 10 & — & — & — &  \\
5 & jvw & 1986 Mar 29-Apr 09 & La Palma INT 2.5m & RCA & 4 & 6 & 8 & 9 & 6 & — &  \\
6 & km & 1986 May 08 & La Palma INT 2.5m & RCA & — & 1 & 2 & — & — & — &  \\
7 & c91ic41 & 1991 Apr 08 & Maunakea CFHT 3.6m & lick1 & — & 2 & 2 & — & 2 & — &  \\
8 & cf91 & 1991 Jul 06-07 & Maunakea CFHT 3.6m & Lick2 & — & 2 & 2 & — & — & — &  \\
9 & saic & 1992 May 25 & Maunakea CFHT 3.6m & HRCam/saic1 & — & — & 16 & 15 & — & — &  \\
10 & h92ic1 & 1992 May 27 & Maunakea CFHT 3.6m & HRCam & — & 7 & — & — & — & — &  \\
11 & cf92 & 1992 Jun 08-09 & Maunakea CFHT 3.6m & RCA4 & — & 3 & — & — & — & — &  \\
12 & bolte & 1994 Apr 13-16 & KPNO 2.1m & t1ka & — & — & 30 & — & 31 & — &  \\
13 & cf94 & 1994 Jun 06 & Maunakea CFHT 3.6m & Loral3 & — & 4 & — & — & 4 & — &  \\
14 & jka & 1995 Mar 27 & La Palma INT 2.5m & TEK3 & — & 3 & 8 & — & — & — &  \\
15 & bond9 & 1997 May 08-10 & KPNO 0.9m & t2ka & — & 4 & 4 & — & 4 & — &  \\
16 & arg & 1997 May 31 & La Palma JKT 1m & TEK2 & — & — & 3 & — & 6 & — &  \\
17 & bond11 & 1998 Mar 21-22 & KPNO 0.9m & t2ka & — & 9 & 9 & — & 9 & — &  \\
18 & int9804 & 1998 Apr 12 & La Palma INT 2.5m & WFC & — & 3 & — & 4 & — & — &  \\
19 & dmd & 1998 Jun 24 & La Palma JKT 1m & TEK4 & — & — & 2 & — & 2 & — &  \\
20 & tng2 & 2000 Feb 04 & La Palma TNG 3.6m & OIG & 2 & 2 & 2 & — & — & — & x  2 \\
21 & int0005 & 2000 May 24-28 & La Palma INT 2.5m & WFC & — & 3 & 3 & — & — & — & x  4 \\
22 & jun00 & 2000 Jun 04 & Maunakea CFHT 3.6m & CFH12K & — & — & 2 & — & — & — & x 12 \\
23 & cf0102 & 2001 Feb 16-17 & Maunakea CFHT 3.6m & CFH12K & — & 15 & 18 & — & 12 & — & x 12 \\
24 & not017 & 2001 Jul 11-15 & La Palma NOT 2.6m & CCD7 & — & 9 & 7 & — & 10 & — &  \\
25 & int0202 & 2002 Feb 03-04 & La Palma INT 2.5m & WFC & — & 112 & 113 & — & — & — & x  4 \\
26 & hannah & 2002 Mar 29 & La Palma JKT 1m & SIT2 & — & 5 & 11 & 10 & — & — &  \\
27 & int1005 & 2010 May 25-30 & La Palma INT 2.5m & WFC & — & 32 & 33 & 33 & 11 & — & x  4 \\
28 & int1202 & 2012 Feb 22-23 & La Palma INT 2.5m & WFC & 16 & — & — & — & — & — & x  4 \\
29 & int1204 & 2012 Apr 23-26 & La Palma INT 2.5m & WFC & 10 & 9 & 9 & — & 6 & — & x  4 \\
30 & int1304 & 2013 Apr 13 & La Palma INT 2.5m & WFC & 10 & — & — & — & — & — & x  4 \\
31 & spm1405a & 2014 May 21 & S Pedro Martir 0.8 & E2V-4290 & 1 & 2 & 2 & 2 & 2 & — &  \\
32 & dahl & 2014 Jun 19-25 & Maria Mitchell 0.4 & Roper PVCAM & — & — & 3 & 3 & — & — &  \\
33 & int1501 & 2015 Jan 30 & La Palma INT 2.5m & WFC & — & 2 & 2 & — & — & — & x  4 \\
34 & int1502 & 2015 Feb 25-27 & La Palma INT 2.5m & WFC & — & 9 & 9 & — & — & — & x  4 \\
35 & int1504 & 2015 Apr 24-27 & La Palma INT 2.5m & WFC & — & 16 & 17 & — & 8 & — & x  4 \\
36 & int1605 & 2016 May 28-Jun 02 & La Palma INT 2.5m & WFC & 1 & 11 & 11 & — & 10 & — & x  4 \\
37 & int1704 & 2017 Apr 03-05 & La Palma INT 2.5m & WFC & — & 6 & 6 & — & 6 & — & x  4 \\
38 & iac80a & 2017 Jun 17-19 & Teide IAC80 0.8m & CAMELOT & 2 & 2 & 2 & 2 & 2 & — &  \\
39 & spm1801b & 2018 Jan 28 & S Pedro Martir 0.8 & E2V-4240 & 2 & 2 & 2 & 2 & 2 & — &  \\
40 & int1802 & 2018 Feb 22 & La Palma INT 2.5m & WFC & 3 & 3 & — & — & — & — & x  4 \\
41 & spm1802 & 2018 Feb 26 & S Pedro Martir 2.1 & E2V-4240 & 3 & 3 & 2 & 3 & 3 & — &  \\
42 & int1805 & 2018 May 20-22 & La Palma INT 2.5m & WFC & 6 & 2 & 6 & 2 & — & — & x  4 \\
43 & int1806 & 2018 Jun 12 & La Palma INT 2.5m & WFC & 2 & 2 & — & 2 & — & — & x  4 \\
44 & int1906 & 2019 Jun 26-29 & La Palma INT 2.5m & WFC & 5 & 2 & — & — & — & — & x  4 \\ 
\hline
\end{tabular}
}
\begin{minipage}{\textwidth}
\vspace{0.1cm}
\small \textbf{Notes}. 1. Observers R. D. McClure and D. A. VandenBerg 2. Observer P. B. Stetson 3. Observer P. B. Stetson 4. Observers J. E. Hesser and D. A. VandenBerg 5. Observer "JVW" 6. Observer "KM" 7. Observers H. Richer and G. Fahlman 8. Observers P. B. Stetson and J. E. Hesser 9. Observers Bolte and Hesser 10. Observers Richer and Buonanno 11. Observers P. B. Stetson and M. Bolte 12. Observer M. Bolte 13. Run ID 94IC15, observers D. A. VandenBerg and P. B. Stetson 14. Observer "JKA" 15. Proposal KP2771, observer H. E. Bond; includes observations in Sloan u filter 16. Observer A. Rosenberg 17. Proposal 98A-0351, observer H. E. Bond 18. Details unavailable 19. Run number 4064, observer "DMD" 20. Observers Ortolani, Bragaglia and "admin" 21. Proposal P14, observer Robert Greimel 22. Run ID 00AC14, observers Stetson and Fahlman 23. Run IDs 01AK1 and 01AF43, observers Park, Sohn and Oh;  R. Ibata and C. Pichon 24. Observer Bruntt 25. Proposal P20, observer G. Gilmore 26. Proposal "ING\_Science," observer Javier Mendez 27. Proposal N5, observer vdWerf 28. Proposal C34, observer Carrera 29. Proposal c70, observer Milone 30. Proposal C143, observer M. Monelli 31. Observers Ricci et al. and Ayala-Michel; data contributed by Raul Michel Murillo 32. Observer E. Dahl 33. Proposals CAT\_S and N22W, observers Oscoz and Vats 34. Proposal C115, observer C. Martinez 35. Proposal N2, observer Henk Hoekstra; proposal C115, observer Clara Martinez 36. Proposal C143, observer Monelli 37. Proposals "(16A)C143" and "CAT\_S," observer M. Monelli 38. Observer M. Monelli 39. Observers Omar and Raul; data contributed by Raul Michel Murillo 40. Proposal C14, observer M. Monelli 41. Observers "ing" and Michel; data contributed by Raul Michel Murillo 42. Proposal C14, observer M. Monelli 43. Proposal C14, observers Monelli and Rusakov 44. Proposal C143, observer Monelli.
\end{minipage}

==> tables/table_2.tex <==

\begin{tabular}{cccccccccccccccc}
Star & Period & Type & <U> & A_U & <B> & A_B & <V> & A_V & <R> & A_R & <I> & A_I & Oo_type & Blazhko & QF \\
 & days &  & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ &  &  &  \\
V1 & 0.52059 & RRab & 15.470 & 0.635 & 16.221 & 0.694 & 15.824 & 0.568 & 15.525 & 0.441 & 15.266 & 0.356 & OoI &  & CCCCC \\
V3 & 0.55820 & RRab & 15.738 & 1.478 & 15.969 & 1.346 & 15.606 & 0.974 & 15.289 & 0.733 & 15.117 & 0.743 & OoII & Bl & CBBBA \\
V4n & 0.58504 & RRab & 15.074 & 0.808 & 15.114 & 0.932 & 14.754 & 0.763 & 14.430 & 0.595 & 14.205 & 0.487 &  &  & CCBBB \\
V5 & 0.50583 & RRab & 15.990 & 1.008 & 16.028 & 1.366 & 15.691 & 1.053 & 15.507 & 0.580 & 15.216 & 0.781 & OoI & Bl & CCCCB \\
V6 & 0.51434 & RRab & 16.012 & 1.419 & 16.045 & 1.268 & 15.693 & 1.130 & 15.498 & 0.715 & 15.243 & 0.813 & OoI &  & BCCCB \\
V7 & 0.49742 & RRab & 15.679 & 0.794 & 15.678 & 0.881 & 15.394 & 0.606 & 15.212 & 0.495 & 15.163 & 0.499 & OoI & Bl & CCCCC \\
V8 & 0.63672 & RRab & 15.684 & 0.648 & 15.735 & 0.851 & 15.273 & 0.585 & 14.913 & 0.401 & 14.566 & 0.236 &  & Bl & CBBCA \\
V9 & 0.55666 & RRab & 16.272 & 0.969 & 15.928 & 1.291 & 15.643 & 1.019 & 15.601 & 0.502 & 15.181 & 0.783 & OoI &  & CCCBC \\
V10 & 0.56955 & RRab & 15.975 & 1.103 & 16.051 & 1.106 & 15.719 & 0.748 & 15.402 & 0.593 & 15.153 & 0.512 & OoI & Bl & BBBAA \\
V11 & 0.50789 & RRab & 15.395 & 1.119 & 16.032 & 1.577 & 15.712 & 1.191 & 15.450 & 1.011 & 15.224 & 0.831 & OoI &  & CBAAB \\
V12 & 0.32557 & RRc & 15.896 & 0.501 & 15.871 & 0.540 & 15.633 & 0.468 & 15.597 & 0.342 & 15.306 & 0.324 &  &  & CCCCC \\
V13 & 0.32350 & RRd & 16.109 & 0.787 & 16.001 & 0.849 & 15.644 & 0.735 & 15.570 & 0.537 & 15.232 & 0.509 &  & Bl & CCCCC \\
V14 & 0.63590 & RRab & 15.910 & 1.315 & 15.901 & 1.278 & 15.550 & 1.004 & 15.169 & 0.882 & 15.054 & 0.556 & OoII & Bl & BCBBA \\
V15 & 0.53009 & RRab & 16.097 & 0.919 & 16.063 & 1.129 & 15.766 & 0.851 & 15.447 & 0.922 & 15.182 & 0.716 & OoI &  & CBBBB \\
V16 & 0.51149 & RRab & 16.054 & 1.465 & 16.103 & 1.460 & 15.766 & 1.134 & 15.546 & 1.008 & 15.270 & 0.827 & OoI &  & ABABB \\
V17 & 0.57616 & RRab & 16.014 & 0.833 & 16.028 & 0.878 & 15.699 & 0.717 & 15.437 & 0.460 & 15.166 & 0.425 & OoI & Bl & CCCAB \\
V18 & 0.51645 & RRab & 16.089 & 1.429 & 16.168 & 1.059 & 15.816 & 0.911 & 15.499 & 0.888 & 15.310 & 0.567 & OoI &  & CBBCB \\
V19 & 0.63197 & RRab & 16.081 & 0.653 & 16.107 & 0.579 & 15.722 & 0.435 & 15.442 & 0.387 & 15.156 & 0.288 & OoI &  & AAABA \\
V20 & 0.49752 & RRab & 15.805 & 1.131 & 15.979 & 1.228 & 15.558 & 1.308 & 15.460 & 0.651 & 15.130 & 0.602 & OoI & Bl & CCCCC \\
V21 & 0.51367 & RRab & 16.026 & 0.934 & 16.158 & 1.180 & 15.776 & 0.875 & 15.620 & 0.493 & 15.203 & 0.452 & OoI &  & CBBCB \\
V22 & 0.48141 & RRab & 15.839 & 1.160 & 16.069 & 1.331 & 15.695 & 1.323 & 15.562 & 0.626 & 15.264 & 0.617 & OoI & Bl & CBBBC \\
V23 & 0.59538 & RRab & 15.865 & 0.961 & 16.055 & 0.944 & 15.681 & 0.763 & 15.291 & 0.550 & 15.143 & 0.460 & OoI & Bl & CBBBB \\
V24 & 0.66340 & RRab & 15.908 & 0.902 & 15.928 & 1.090 & 15.560 & 0.825 & 15.213 & 0.434 & 15.027 & 0.431 & OoII & Bl & CBBBB \\
V25 & 0.48006 & RRab & 16.010 & 1.426 & 16.157 & 1.312 & 15.713 & 1.116 & 15.532 & 1.050 & 15.264 & 0.683 & OoI &  & BCBBB \\
V26 & 0.59774 & RRab & 15.922 & 1.184 & 15.961 & 1.177 & 15.618 & 0.906 & 15.374 & 0.788 & 15.089 & 0.668 & OoII &  & ABAAA \\
V27 & 0.57906 & RRab & 15.964 & 1.066 & 16.018 & 1.102 & 15.661 & 0.840 & 15.401 & 0.781 & 15.145 & 0.568 & OoI &  & ABBBB \\
V28 & 0.47064 & RRab & 15.934 & 1.223 & 15.960 & 1.378 & 15.690 & 1.053 & 15.511 & 0.793 & 15.247 & 0.640 & OoI & Bl & CCCBB \\
V29 & 0.47178 & RRab & 15.773 & 1.060 & 15.895 & 1.171 & 15.576 & 0.970 & 15.405 & 0.649 & 15.193 & 0.653 &  &  & CCCCC \\
V30 & 0.51209 & RRab & 16.199 & 1.018 & 15.978 & 1.254 & 15.633 & 1.018 & 15.421 & 0.846 & 15.171 & 0.696 &  &  & BBBAA \\
V31 & 0.58073 & RRab & 15.830 & 1.410 & 15.890 & 1.377 & 15.570 & 1.140 & 15.163 & 0.805 & 15.085 & 0.710 & OoII &  & BBBBB \\
V32 & 0.49535 & RRab & 16.093 & 0.896 & 15.930 & 1.382 & 15.613 & 1.100 & 15.513 & 0.627 & 15.106 & 0.698 & OoI &  & BBAAA \\
V33 & 0.52525 & RRab & 15.832 & 1.080 & 15.994 & 1.138 & 15.671 & 0.932 & 15.552 & 0.652 & 15.174 & 0.610 & OoI & Bl & CCCBB \\
V34 & 0.55910 & RRab & 16.012 & 0.746 & 16.072 & 0.903 & 15.718 & 0.743 & 15.372 & 0.694 & 15.203 & 0.440 & OoI & Bl & CBBCB \\
V35 & 0.52976 & RRab & 15.919 & 1.208 & 16.040 & 1.354 & 15.723 & 1.110 & 15.465 & 0.730 & 15.242 & 0.633 & OoI & Bl & CBBCC \\
V36 & 0.54559 & RRab & 15.931 & 1.402 & 16.075 & 1.285 & 15.729 & 1.011 & 15.341 & 0.556 & 15.206 & 0.752 & OoI &  & CBBBB \\
V37 & 0.32664 & RRc & 15.927 & 0.604 & 15.898 & 0.651 & 15.669 & 0.564 & 15.479 & 0.423 & 15.290 & 0.390 &  &  & BCCBC \\
V38 & 0.55801 & RRab & 15.995 & 1.253 & 16.066 & 0.972 & 15.716 & 0.706 & 15.353 & 0.496 & 15.222 & 0.471 & OoI & Bl & CCCBB \\
V39 & 0.58707 & RRab & 16.078 & 0.696 & 16.023 & 0.906 & 15.669 & 0.710 & 15.459 & 0.422 & 15.169 & 0.503 & OoI & Bl & CCCAB \\
V40 & 0.55154 & RRab & 16.042 & 1.184 & 16.104 & 1.207 & 15.738 & 0.945 & 15.335 & 0.882 & 15.240 & 0.600 & OoI &  & BBBBB \\
V41 & 0.48509 & RRab & 16.014 & 1.435 & 16.010 & 1.511 & 15.626 & 1.067 & 15.476 & 0.862 & 15.275 & 0.586 & OoI & Bl & CCCBC \\
V42 & 0.59008 & RRab & 15.787 & 1.240 & 15.750 & 1.338 & 15.457 & 1.009 & 15.432 & 0.595 & 15.059 & 0.765 & OoII &  & CCCBB \\
V43 & 0.54052 & RRab & 16.022 & 1.397 & 16.032 & 1.337 & 15.711 & 1.050 & 15.458 & 0.823 & 15.189 & 0.674 &  & Bl & BBAAA \\
V44 & 0.36810 & RRd & 15.775 & 0.821 & 16.051 & 0.885 & 15.606 & 0.767 & 15.113 & 0.560 & 15.271 & 0.531 &  & Bl & CCCCC \\
V45 & 0.53691 & RRab & 16.248 & 0.969 & 16.229 & 1.036 & 15.784 & 0.849 & 15.570 & 0.725 & 15.291 & 0.557 & OoI & Bl & CBBAC \\
V46 & 0.61339 & RRab & 16.036 & 0.758 & 16.108 & 0.688 & 15.712 & 0.500 & 15.425 & 0.374 & 15.149 & 0.361 & OoI &  & BBBAA \\
V47 & 0.57257 & RRab & 15.927 & 0.890 & 15.923 & 0.952 & 15.594 & 0.780 & 15.506 & 0.448 & 15.192 & 0.531 & OoI & Bl & CCCBC \\
V48 & 0.62784 & RRab & 15.893 & 0.597 & 15.935 & 0.685 & 15.544 & 0.506 & 15.245 & 0.392 & 14.959 & 0.378 & OoI? & Bl & CCBBB \\
V49 & 0.54821 & RRab & 15.938 & 1.113 & 15.920 & 1.105 & 15.544 & 0.944 & 15.409 & 0.652 & 15.170 & 0.628 & OoI & Bl & CCCAB \\
V50 & 0.51310 & RRab & 16.096 & 1.300 & 16.063 & 1.268 & 15.672 & 1.117 & 15.513 & 0.767 & 15.257 & 0.590 & OoI & Bl & CCCAB \\
V51 & 0.58397 & RRab & 16.001 & 0.940 & 16.042 & 1.035 & 15.691 & 0.811 & 15.391 & 0.592 & 15.150 & 0.585 & OoI &  & BBBAA \\
V52 & 0.51624 & RRab & 16.188 & 1.204 & 15.965 & 1.249 & 15.674 & 0.899 & 15.459 & 0.631 & 15.247 & 0.802 & OoI & Bl & CCCCC \\
V53 & 0.50488 & RRab & 16.298 & 0.435 & 16.358 & 0.469 & 15.994 & 0.396 & 15.656 & 0.249 & 15.286 & 0.248 & OoI &  & CCCCC \\
V54 & 0.50620 & RRab & 16.056 & 0.836 & 16.170 & 0.942 & 15.779 & 0.727 & 15.523 & 0.712 & 15.239 & 0.420 & OoI & Bl & CCCBC \\
V55 & 0.52983 & RRab & 16.150 & 1.209 & 16.013 & 1.094 & 15.683 & 0.895 & 15.447 & 0.774 & 15.228 & 0.717 & OoI &  & BCBCB \\
V56 & 0.32960 & RRc & 15.874 & 0.553 & 15.926 & 0.579 & 15.648 & 0.468 & 15.469 & 0.404 & 15.278 & 0.304 &  &  & BBABA \\
V57 & 0.51218 & RRab & 16.143 & 1.099 & 16.116 & 1.214 & 15.753 & 0.968 & 15.564 & 0.779 & 15.184 & 0.583 & OoI &  & CBABB \\
V58 & 0.51705 & RRab & 15.999 & 1.600 & 15.858 & 1.455 & 15.619 & 1.151 & 15.409 & 0.685 & 15.190 & 0.827 & OoI &  & CCBAB \\
V59 & 0.58883 & RRab & 16.062 & 0.970 & 16.076 & 0.927 & 15.693 & 0.744 & 15.459 & 0.543 & 15.182 & 0.466 & OoI & Bl & ABBAA \\
V60 & 0.70773 & RRab & 15.956 & 0.844 & 15.949 & 0.845 & 15.566 & 0.646 & 15.344 & 0.603 & 15.012 & 0.415 & OoII &  & BABAA \\
V61 & 0.52089 & RRab & 16.051 & 1.097 & 16.119 & 1.004 & 15.738 & 0.732 & 15.589 & 0.434 & 15.196 & 0.571 &  &  & BBABB \\
V62 & 0.65240 & RRab & 16.002 & 0.675 & 16.045 & 0.668 & 15.645 & 0.490 & 15.384 & 0.515 & 15.079 & 0.323 & OoI & Bl & AAAAA \\
V63 & 0.57040 & RRab & 16.025 & 1.215 & 16.076 & 1.232 & 15.722 & 0.889 & 15.523 & 0.580 & 15.189 & 0.586 & OoI & Bl & BCCCB \\
V64 & 0.60546 & RRab & 16.066 & 0.841 & 16.101 & 0.945 & 15.714 & 0.711 & 15.461 & 0.607 & 15.158 & 0.444 & OoI &  & BAAAA \\
V65 & 0.66716 & RRab & 16.057 & 0.999 & 15.959 & 1.156 & 15.582 & 0.946 & 15.377 & 0.527 & 15.010 & 0.592 & OoII &  & CBCCC \\
V66 & 0.62019 & RRab & 16.010 & 0.705 & 16.060 & 0.784 & 15.657 & 0.615 & 15.412 & 0.461 & 15.125 & 0.366 & OoI & Bl & CCCBB \\
V67 & 0.56833 & RRab & 16.041 & 0.704 & 16.113 & 0.854 & 15.720 & 0.746 & 15.479 & 0.617 & 15.193 & 0.476 & OoI & Bl & CCBBB \\
V68 & 0.36053 & RRd & 15.932 & 0.675 & 15.823 & 0.728 & 15.528 & 0.630 & 15.411 & 0.460 & 15.222 & 0.436 &  &  & CCCCC \\
V69 & 0.56662 & RRab & 16.113 & 1.087 & 16.089 & 1.157 & 15.730 & 0.899 & 15.448 & 0.698 & 15.193 & 0.545 & OoI &  & BBBAA \\
V70 & 0.48606 & RRc & 15.576 & 0.360 & 15.675 & 0.425 & 15.368 & 0.340 & 15.168 & 0.253 & 14.921 & 0.232 &  & Bl & CBBAB \\
V71 & 0.54905 & RRab & 15.958 & 1.132 & 16.083 & 1.166 & 15.725 & 0.905 & 15.511 & 0.705 & 15.181 & 0.531 & OoI & Bl & BAAAA \\
V72 & 0.45608 & RRab & 15.839 & 1.487 & 15.945 & 1.461 & 15.716 & 1.190 & 15.293 & 0.882 & 15.332 & 0.726 & OoI &  & CCCCA \\
V73 & 0.67348 & RRab & 16.001 & 0.430 & 16.073 & 0.350 & 15.671 & 0.272 & 15.348 & 0.227 & 15.074 & 0.155 & OoI & Bl & BAABB \\
V74 & 0.49216 & RRab & 16.070 & 1.528 & 16.060 & 1.633 & 15.671 & 1.350 & 15.570 & 0.850 & 15.285 & 0.713 & OoI &  & BCBBC \\
V75 & 0.31408 & RRc & 15.913 & 0.554 & 15.936 & 0.578 & 15.686 & 0.489 & 15.518 & 0.357 & 15.303 & 0.338 &  &  & BCCAA \\
V76 & 0.50176 & RRab & 15.938 & 1.591 & 16.049 & 1.518 & 15.720 & 1.203 & 15.331 & 0.582 & 15.266 & 0.724 & OoI &  & BBBCB \\
V77 & 0.45935 & RRab & 16.397 & 0.855 & 15.999 & 1.133 & 15.805 & 1.015 & 15.783 & 0.586 & 15.446 & 0.559 & OoI & Bl & CCCCC \\
V78 & 0.61191 & RRab & 15.855 & 0.970 & 16.017 & 0.812 & 15.667 & 0.607 & 15.413 & 0.395 & 15.086 & 0.381 & OoII? & Bl & CBCBB \\
V79 & 0.48326 & RRab & 16.161 & 0.893 & 16.187 & 0.973 & 15.910 & 0.790 & 15.513 & 0.469 & 15.337 & 0.466 & OoI & Bl & CCCCC \\
V80 & 0.52906 & RRab & 16.022 & 0.809 & 16.254 & 0.899 & 15.739 & 0.852 & 15.401 & 0.572 & 15.293 & 0.521 & OoI & Bl & CCCBB \\
V81 & 0.52912 & RRab & 15.812 & 1.393 & 16.132 & 1.199 & 15.706 & 1.083 & 15.450 & 0.675 & 15.216 & 0.730 & OoI &  & CBAAA \\
V82 & 0.52454 & RRab & 16.035 & 1.438 & 16.078 & 1.355 & 15.744 & 1.061 & 15.475 & 0.948 & 15.228 & 0.719 & OoI &  & BCCAB \\
V83 & 0.50127 & RRab & 16.092 & 0.979 & 16.141 & 1.320 & 15.766 & 0.952 & 15.692 & 0.512 & 15.287 & 0.859 & OoI &  & CBBBC \\
V84 & 0.59573 & RRab & 15.985 & 1.018 & 16.064 & 0.933 & 15.704 & 0.698 & 15.394 & 0.633 & 15.145 & 0.486 & OoI &  & BBAAA \\
V85 & 0.35581 & RRc & 15.835 & 0.538 & 15.740 & 0.546 & 15.512 & 0.430 & 15.360 & 0.314 & 15.154 & 0.297 &  &  & CCBCB \\
V86 & 0.29266 & RRc & 15.948 & 0.484 & 15.899 & 0.645 & 15.695 & 0.498 & 15.490 & 0.330 & 15.327 & 0.313 &  &  & CBBCA \\
V87 & 0.35748 & RRd & 15.846 & 0.510 & 15.871 & 0.550 & 15.593 & 0.476 & 15.299 & 0.348 & 15.146 & 0.329 &  &  & CCCBB \\
V88 & 0.29875 & RRc & 15.940 & 0.703 & 15.922 & 0.758 & 15.701 & 0.657 & 15.415 & 0.480 & 15.370 & 0.454 &  &  & CCCCC \\
V89 & 0.54848 & RRab & 16.042 & 1.107 & 16.004 & 1.309 & 15.663 & 0.999 & 15.388 & 0.743 & 15.139 & 0.624 & OoI &  & BBAAA \\
V90 & 0.51703 & RRab & 16.000 & 1.370 & 16.078 & 1.356 & 15.782 & 1.055 & 15.543 & 0.850 & 15.234 & 0.751 & OoI &  & BBBBB \\
V91 & 0.53011 & RRab & 15.859 & 1.018 & 16.066 & 1.168 & 15.702 & 0.804 & 15.409 & 0.770 & 15.202 & 0.479 & OoI & Bl & CBBCC \\
V92 & 0.50355 & RRab & 15.964 & 0.874 & 16.113 & 0.814 & 15.783 & 0.677 & 15.481 & 0.448 & 15.415 & 0.447 & OoI & Bl & CCCCC \\
V93 & 0.60230 & RRab & 15.935 & 0.830 & 16.108 & 0.896 & 15.718 & 0.667 & 15.529 & 0.644 & 15.183 & 0.502 & OoI &  & CCCAB \\
V94 & 0.52370 & RRab & 16.335 & 0.899 & 15.948 & 1.042 & 15.720 & 0.848 & 15.493 & 0.546 & 15.298 & 0.541 & OoI &  & CCCCC \\
V96 & 0.49941 & RRab & 15.624 & 0.769 & 16.234 & 0.985 & 15.858 & 0.813 & 15.529 & 0.705 & 15.377 & 0.699 & OoI &  & CBBBB \\
V97 & 0.33493 & RRc & 16.059 & 0.392 & 15.976 & 0.508 & 15.710 & 0.409 & 15.518 & 0.343 & 15.311 & 0.254 &  &  & BBBAB \\
V99 & 0.35543 & RRd & 15.760 & 0.526 & 15.913 & 0.567 & 15.665 & 0.491 & 15.375 & 0.391 & 15.158 & 0.340 &  & Bl & CCCBC \\
V100 & 0.61881 & RRab & 15.988 & 0.657 & 16.177 & 0.583 & 15.744 & 0.502 & 15.452 & 0.489 & 15.101 & 0.273 & OoI &  & CBBAC \\
V101 & 0.64389 & RRab & 16.013 & 0.645 & 16.065 & 0.652 & 15.669 & 0.537 & 15.370 & 0.364 & 15.110 & 0.359 & OoI & Bl & BBABA \\
V104 & 0.56993 & RRab & 15.832 & 1.424 & 15.917 & 1.421 & 15.610 & 1.127 & 15.362 & 0.852 & 15.110 & 0.706 & OoII & Bl & CBBAB \\
V105 & 0.28775 & RRc & 15.866 & 0.408 & 15.819 & 0.440 & 15.619 & 0.381 & 15.440 & 0.287 & 15.334 & 0.264 &  &  & BCCBB \\
V106 & 0.53725 & RRab & 16.016 & 0.745 & 16.040 & 0.876 & 15.695 & 0.661 & 15.492 & 0.379 & 15.234 & 0.444 & OoI & Bl & CCCBC \\
V107 & 0.30903 & RRc & 16.089 & 0.490 & 15.874 & 0.528 & 15.664 & 0.458 & 15.312 & 0.334 & 15.342 & 0.317 &  &  & CCCCC \\
V108 & 0.51961 & RRab & 16.080 & 1.414 & 16.084 & 1.376 & 15.764 & 1.079 & 15.546 & 0.646 & 15.273 & 0.745 & OoI &  & BBACA \\
V109 & 0.53392 & RRab & 16.109 & 1.270 & 16.064 & 1.422 & 15.706 & 1.057 & 15.295 & 0.752 & 15.202 & 0.754 & OoI &  & BBBBA \\
V110 & 0.53546 & RRab & 16.034 & 0.970 & 16.009 & 1.127 & 15.671 & 0.924 & 15.375 & 0.688 & 15.168 & 0.617 & OoI & Bl & CCCBB \\
V111 & 0.51019 & RRab & 15.866 & 1.108 & 16.070 & 1.065 & 15.738 & 0.923 & 15.345 & 0.566 & 15.246 & 0.557 & OoI & Bl & CBBBA \\
V113 & 0.51300 & RRab & 16.200 & 1.095 & 15.981 & 1.497 & 15.674 & 1.196 & 15.502 & 0.574 & 15.153 & 0.654 & OoI &  & CCCCB \\
V114 & 0.59772 & RRab & 15.981 & 1.012 & 16.092 & 0.972 & 15.693 & 0.780 & 15.467 & 0.539 & 15.154 & 0.456 & OoI & Bl & BCBAB \\
V115 & 0.51335 & RRab & 15.821 & 1.352 & 16.039 & 1.527 & 15.710 & 1.188 & 15.387 & 0.736 & 15.236 & 0.742 & OoI &  & CAACA \\
V116 & 0.51481 & RRab & 16.074 & 1.338 & 15.999 & 1.326 & 15.696 & 1.040 & 15.499 & 0.807 & 15.274 & 0.741 & OoI &  & CCBBB \\
V117 & 0.60054 & RRab & 16.076 & 1.100 & 15.994 & 1.209 & 15.649 & 0.836 & 15.427 & 0.675 & 15.125 & 0.583 & OoI & Bl & CCBAB \\
V118 & 0.49940 & RRab & 16.476 & 1.150 & 15.968 & 1.538 & 15.737 & 1.212 & 15.728 & 0.668 & 15.278 & 0.809 &  &  & CCCCB \\
V119 & 0.51835 & RRab & 16.177 & 1.106 & 15.910 & 1.269 & 15.673 & 0.969 & 15.331 & 0.566 & 15.242 & 0.666 & OoI & Bl & CCCCB \\
V120 & 0.64014 & RRab & 16.048 & 0.547 & 16.091 & 0.583 & 15.699 & 0.404 & 15.399 & 0.241 & 15.128 & 0.302 & OoI &  & BBBBA \\
V121 & 0.53521 & RRab & 16.022 & 1.320 & 16.039 & 1.242 & 15.708 & 0.928 & 15.466 & 0.640 & 15.167 & 0.656 & OoI & Bl & CCBAB \\
V122 & 0.51093 & RRab & 16.196 & 1.048 & 16.114 & 1.301 & 15.711 & 1.166 & 15.657 & 0.922 & 15.255 & 0.661 &  &  & CCCCB \\
V123 & 0.54548 & RRab & 16.040 & 1.267 & 15.981 & 1.306 & 15.659 & 1.046 & 15.434 & 0.610 & 15.194 & 0.719 & OoI &  & CBCAA \\
V124 & 0.75244 & RRab & 15.920 & 0.517 & 15.967 & 0.459 & 15.566 & 0.356 & 15.268 & 0.290 & 14.982 & 0.229 & OoII &  & BAAAA \\
V125 & 0.34982 & RRd & 15.900 & 0.486 & 15.963 & 0.496 & 15.707 & 0.368 & 15.487 & 0.288 & 15.225 & 0.255 &  &  & CCBBB \\
V126 & 0.34840 & RRc & 15.951 & 0.428 & 15.972 & 0.462 & 15.686 & 0.400 & 15.440 & 0.193 & 15.244 & 0.277 &  & Bl & CCCBC \\
V128 & 0.29204 & RRc & 15.880 & 0.540 & 15.878 & 0.651 & 15.654 & 0.535 & 15.551 & 0.363 & 15.311 & 0.344 &  &  & CBBBA \\
V130 & 0.55904 & RRab & 15.851 & 0.829 & 15.975 & 0.861 & 15.603 & 0.710 & 15.384 & 0.474 & 15.107 & 0.421 & OoI & Bl & CCBBC \\
V131 & 0.29769 & RRc & 15.840 & 0.558 & 15.865 & 0.631 & 15.640 & 0.506 & 15.520 & 0.488 & 15.277 & 0.351 &  &  & CBAAA \\
V132 & 0.33986 & RRc & 15.814 & 0.467 & 15.893 & 0.453 & 15.621 & 0.380 & 15.509 & 0.278 & 15.209 & 0.263 &  &  & BCBCB \\
V133 & 0.55073 & RRab & 16.187 & 0.996 & 15.906 & 1.064 & 15.725 & 0.977 & 15.523 & 0.600 & 15.198 & 0.587 & OoI & Bl & CCBAB \\
V134 & 0.61806 & RRab & 15.943 & 0.798 & 16.049 & 0.784 & 15.655 & 0.574 & 15.454 & 0.482 & 15.102 & 0.392 &  &  & BAAAA \\
V135 & 0.56839 & RRab & 15.709 & 0.899 & 16.022 & 1.168 & 15.661 & 0.885 & 15.393 & 0.585 & 15.129 & 0.608 & OoI & Bl & CBBBA \\
V136 & 0.61718 & RRab & 15.793 & 0.800 & 15.909 & 0.797 & 15.520 & 0.632 & 15.203 & 0.628 & 14.956 & 0.405 &  &  & CBBBA \\
V137 & 0.57515 & RRab & 15.837 & 1.114 & 15.986 & 1.088 & 15.620 & 0.879 & 15.315 & 0.486 & 15.099 & 0.481 & OoI &  & BBAAA \\
V139 & 0.55999 & RRab & 15.784 & 1.408 & 15.849 & 1.347 & 15.484 & 1.098 & 15.217 & 1.036 & 15.044 & 0.822 &  &  & BBBBA \\
V140 & 0.33314 & RRc & 15.698 & 0.475 & 15.731 & 0.529 & 15.499 & 0.418 & 15.264 & 0.352 & 15.132 & 0.272 &  & Bl & CBBBB \\
V142 & 0.56863 & RRab & 15.974 & 1.198 & 16.094 & 1.219 & 15.710 & 0.968 & 15.477 & 0.826 & 15.203 & 0.644 & OoI &  & BBAAA \\
V143 & 0.59654 & RRab & 15.473 & 0.980 & 15.895 & 0.848 & 15.435 & 0.703 & 15.202 & 0.481 & 14.809 & 0.503 & OoII & Bl & CCBBB \\
V144 & 0.59679 & RRab & 15.946 & 0.583 & 15.994 & 0.618 & 15.601 & 0.506 & 15.281 & 0.346 & 15.058 & 0.344 &  &  & CBABA \\
V145 & 0.51449 & RRab & 15.627 & 0.998 & 15.755 & 1.116 & 15.408 & 0.841 & 15.045 & 0.533 & 14.875 & 0.576 &  &  & CBACB \\
V146 & 0.50220 & RRab & 15.754 & 1.079 & 15.972 & 1.178 & 15.659 & 0.915 & 15.579 & 0.894 & 15.192 & 0.669 & OoI &  & CCBBB \\
V147 & 0.34648 & RRc & 15.836 & 0.475 & 15.954 & 0.514 & 15.657 & 0.444 & 15.448 & 0.424 & 15.260 & 0.307 &  &  & CCBBB \\
V148 & 0.46727 & RRab & 16.158 & 1.314 & 16.200 & 1.654 & 15.808 & 1.497 & 15.453 & 1.460 & 15.354 & 1.030 &  &  & CCBBB \\
V149 & 0.54818 & RRab & 16.099 & 0.952 & 15.931 & 1.298 & 15.622 & 0.971 & 15.381 & 0.595 & 15.140 & 0.520 &  & Bl & BBBAA \\
V150 & 0.52392 & RRab & 15.744 & 1.246 & 16.028 & 1.252 & 15.674 & 1.000 & 15.529 & 0.743 & 15.211 & 0.638 & OoI & Bl & CBBBB \\
V151 & 0.51682 & RRab & 15.630 & 0.913 & 16.038 & 1.009 & 15.660 & 0.825 & 15.507 & 0.555 & 15.148 & 0.571 &  & Bl & CBBCB \\
V152 & 0.32613 & RRc & 15.712 & 0.480 & 15.697 & 0.517 & 15.493 & 0.448 & 15.328 & 0.327 & 15.179 & 0.310 &  &  & CBBAB \\
V155 & 0.33232 & RRc & 15.758 & 0.702 & 15.793 & 0.757 & 15.544 & 0.656 & 15.298 & 0.479 & 15.177 & 0.454 &  &  & CCCBB \\
V156 & 0.53199 & RRab & 15.776 & 1.204 & 15.836 & 1.280 & 15.501 & 0.988 & 15.225 & 0.805 & 15.032 & 0.626 &  &  & ABAAA \\
V157 & 0.54284 & RRab & 15.465 & 0.659 & 16.111 & 0.710 & 15.634 & 0.610 & 15.144 & 0.381 & 14.920 & 0.386 &  & Bl & CBBCC \\
V159 & 0.53380 & RRab & 15.473 & 0.899 & 15.662 & 0.993 & 15.138 & 0.853 & 15.015 & 0.567 & 14.737 & 0.532 &  & Bl & CCCBB \\
V160 & 0.65732 & RRab & 15.729 & 1.044 & 15.863 & 1.109 & 15.500 & 0.924 & 15.329 & 0.617 & 15.009 & 0.576 &  & Bl & CBBBB \\
V161 & 0.52515 & RRab & 15.853 & 1.096 & 15.858 & 1.314 & 15.525 & 1.002 & 15.131 & 0.653 & 14.948 & 0.639 &  & Bl & CCCBB \\
V165 & 0.48363 & RRab & 16.014 & 1.260 & 15.790 & 1.503 & 15.452 & 1.325 & 15.516 & 0.747 & 15.139 & 0.720 &  & Bl & CCCAB \\
V166 & 0.32266 & RRd & 16.140 & 0.716 & 15.960 & 0.772 & 15.693 & 0.669 & 15.494 & 0.488 & 15.262 & 0.463 &  & Bl & CCCCC \\
V167 & 0.64396 & RRab & 15.967 & 0.531 & 16.078 & 0.515 & 15.687 & 0.383 & 15.380 & 0.407 & 15.119 & 0.276 & OoI & Bl & CBBBB \\
V168 & 0.27594 & RRc & 15.734 & 0.532 & 15.796 & 0.574 & 15.582 & 0.497 & 15.397 & 0.363 & 15.204 & 0.344 &  & Bl & CCBBB \\
V170 & 0.43230 & RRc & 15.506 & 0.475 & 15.480 & 0.513 & 15.259 & 0.444 & 15.145 & 0.324 & 14.855 & 0.307 &  &  & CCCBC \\
V171 & 0.30506 & RRc & 15.787 & 0.658 & 15.723 & 0.709 & 15.483 & 0.614 & 15.401 & 0.449 & 15.218 & 0.425 &  &  & CBBBB \\
V172 & 0.54229 & RRab & 16.205 & 0.374 & 15.711 & 0.760 & 15.602 & 0.557 & 15.716 & 0.424 & 15.306 & 0.407 &  &  & CCCBC \\
V173 & 0.60700 & RRab & 15.598 & 1.242 & 15.797 & 1.411 & 15.356 & 1.104 & 15.244 & 1.129 & 14.959 & 0.734 &  &  & CBBBB \\
V174 & 0.59130 & RRab & 16.010 & 0.770 & 16.036 & 0.823 & 15.642 & 0.674 & 15.406 & 0.686 & 15.073 & 0.463 &  & Bl & CCCBB \\
V175 & 0.56970 & RRab & 15.988 & 1.169 & 16.075 & 1.146 & 15.714 & 0.815 & 15.406 & 0.689 & 15.163 & 0.558 &  &  & BAAAA \\
V176 & 0.53962 & RRab & 16.065 & 0.794 & 15.989 & 0.846 & 15.693 & 0.692 & 15.536 & 0.706 & 15.222 & 0.469 &  & Bl & CCBAB \\
V177 & 0.34835 & RRc & 15.732 & 0.582 & 15.728 & 0.581 & 15.509 & 0.459 & 15.350 & 0.353 & 15.140 & 0.318 &  &  & BBBAB \\
V178 & 0.26696 & RRc & 15.847 & 0.396 & 15.862 & 0.427 & 15.680 & 0.370 & 15.563 & 0.270 & 15.380 & 0.256 &  &  & CCCCC \\
V180 & 0.60910 & RRab & 15.772 & 0.681 & 16.007 & 0.732 & 15.587 & 0.627 & 15.314 & 0.420 & 15.023 & 0.405 &  &  & BBBAA \\
V181 & 0.66385 & RRab & 15.699 & 0.859 & 15.886 & 0.905 & 15.478 & 0.743 & 15.037 & 0.753 & 14.863 & 0.490 &  &  & CBBBA \\
V184 & 0.53123 & RRab & 15.867 & 1.142 & 15.913 & 1.289 & 15.619 & 1.019 & 15.489 & 0.690 & 15.179 & 0.701 &  & Bl & CBBBB \\
V186 & 0.66325 & RRab & 15.873 & 0.563 & 15.975 & 0.588 & 15.591 & 0.479 & 15.191 & 0.330 & 15.013 & 0.358 &  & Bl & CBBCB \\
V187 & 0.58628 & RRab & 15.951 & 1.199 & 16.030 & 1.065 & 15.643 & 0.761 & 15.411 & 0.658 & 15.152 & 0.539 &  &  & BBBAB \\
V188 & 0.26652 & RRc & 15.880 & 0.429 & 15.902 & 0.463 & 15.693 & 0.401 & 15.604 & 0.293 & 15.392 & 0.278 &  &  & CBBAA \\
V189 & 0.61294 & RRab & 15.782 & 1.012 & 15.946 & 0.901 & 15.503 & 0.737 & 15.311 & 0.601 & 14.919 & 0.409 &  &  & BBBAA \\
V190 & 0.52280 & RRab & 15.947 & 1.356 & 16.013 & 1.396 & 15.673 & 1.082 & 15.277 & 0.892 & 15.196 & 0.688 &  &  & BBBBA \\
V191 & 0.51919 & RRab & 15.815 & 1.356 & 16.033 & 1.457 & 15.678 & 1.266 & 15.615 & 0.742 & 15.257 & 0.654 &  & Bl & BBBAB \\
V192 & 0.49740 & RRab & 14.542 & 0.615 & 14.757 & 0.657 & 14.149 & 0.538 & 13.829 & 0.368 & 13.367 & 0.356 &  & Bl & BBBCB \\
V193 & 0.74787 & RRab & 15.361 & 1.015 & 15.498 & 1.037 & 15.129 & 0.892 & 14.897 & 0.893 & 14.637 & 0.645 &  &  & BBBAB \\
V194 & 0.48920 & RRab & 15.396 & 1.142 & 15.567 & 1.181 & 15.091 & 0.844 & 14.808 & 0.959 & 14.543 & 0.615 &  &  & BBBAA \\
V195 & 0.64392 & RRab & 15.845 & 0.902 & 15.877 & 1.031 & 15.568 & 0.603 & 15.287 & 0.551 & 14.997 & 0.555 &  & Bl & CCCCC \\
V197 & 0.49990 & RRab & 16.113 & 1.238 & 16.086 & 1.443 & 15.718 & 1.175 & 15.194 & 0.719 & 15.275 & 0.717 &  &  & BBBCC \\
V200 & 0.36100 & RRd & 15.393 & 0.821 & 15.820 & 0.885 & 15.500 & 0.913 & 15.256 & 0.560 & 14.985 & 0.531 &  &  & CCCBB \\
V201 & 0.54053 & RRab & 15.186 & 0.948 & 15.571 & 1.079 & 15.142 & 0.882 & 14.836 & 0.574 & 14.828 & 0.577 &  & Bl & BBBBC \\
V202 & 0.77357 & RRab & 15.925 & 0.225 & 15.973 & 0.193 & 15.563 & 0.138 & 15.269 & 0.153 & 14.974 & 0.096 & OoII &  & BBACA \\
V203 & 0.28980 & RRc & 15.838 & 0.189 & 15.758 & 0.204 & 15.599 & 0.177 & 15.428 & 0.129 & 15.299 & 0.122 &  & Bl & CCBCB \\
V205 & 0.63690 & RRab & 16.035 & 0.648 & 16.128 & 0.483 & 15.716 & 0.421 &  &  & 15.152 & 0.236 & OoI &  & CCCBB \\
V207 & 0.34531 & RRc & 15.698 & 0.609 & 15.816 & 0.657 & 15.526 & 0.569 & 15.264 & 0.433 & 15.079 & 0.394 &  &  & BCCBB \\
V208 & 0.33839 & RRc & 15.769 & 0.429 & 15.801 & 0.476 & 15.511 & 0.401 & 15.254 & 0.293 & 15.026 & 0.278 &  &  & BBBBA \\
V209 & 0.34828 & RRc & 15.818 & 0.520 & 15.799 & 0.561 & 15.556 & 0.486 & 15.373 & 0.427 & 15.181 & 0.336 &  &  & CCCBB \\
V210 & 0.35295 & RRc & 15.883 & 0.581 & 15.919 & 0.627 & 15.668 & 0.543 & 15.438 & 0.460 & 15.243 & 0.376 &  &  & CBBAB \\
V211 & 0.55820 & RRab & 15.908 & 1.182 & 16.125 & 1.106 & 15.721 & 0.943 & 15.256 & 0.605 & 15.295 & 0.624 &  & Bl & CCBCB \\
V212 & 0.54220 & RRab & 15.827 & 1.069 & 15.915 & 1.177 & 15.586 & 0.966 & 15.389 & 0.732 & 15.113 & 0.558 &  & Bl & BBAAA \\
V213 & 0.30000 & RRc & 15.615 & 0.487 & 15.621 & 0.526 & 15.347 & 0.455 & 15.171 & 0.333 & 14.966 & 0.315 &  &  & CCBBB \\
V214 & 0.53951 & RRab & 15.839 & 1.430 & 16.016 & 1.253 & 15.649 & 1.026 & 15.412 & 0.671 & 15.128 & 0.666 &  & Bl & CBBBB \\
V215 & 0.52870 & RRab & 15.594 & 0.914 & 15.708 & 0.991 & 15.412 & 0.812 & 15.244 & 0.533 & 15.085 & 0.536 &  &  & CCCCB \\
V216 & 0.34648 & RRc & 15.745 & 0.533 & 15.828 & 0.575 & 15.560 & 0.498 & 15.380 & 0.363 & 15.161 & 0.344 &  &  & ABBBA \\
V217 & 0.52836 & RRab & 15.476 & 1.406 & 15.728 & 1.194 & 15.387 & 0.982 & 15.264 & 0.942 & 14.948 & 0.679 &  &  & BBAAA \\
V218 & 0.54487 & RRab & 15.920 & 0.982 & 15.992 & 1.020 & 15.630 & 0.843 & 15.414 & 0.510 & 15.067 & 0.562 & OoI & Bl & BBBAA \\
V219 & 0.61361 & RRab & 15.996 & 0.884 & 16.043 & 0.940 & 15.674 & 0.763 & 15.454 & 0.445 & 15.104 & 0.508 &  & Bl & BBBAB \\
V220 & 0.60011 & RRab & 15.954 & 0.658 & 15.988 & 0.899 & 15.606 & 0.793 & 15.354 & 0.698 & 14.966 & 0.424 &  & Bl & BBBAA \\
V221 & 0.37877 & RRc & 15.353 & 0.615 & 15.437 & 0.663 & 15.190 & 0.574 & 15.031 & 0.419 & 14.831 & 0.397 &  &  & BBBBB \\
V222 & 0.59674 & RRab & 15.786 & 0.871 & 15.939 & 1.036 & 15.558 & 0.732 & 15.175 & 0.601 & 15.041 & 0.418 & OoI &  & BBABB \\
V223 & 0.32923 & RRc & 15.632 & 0.772 & 15.684 & 0.833 & 15.433 & 0.721 & 15.355 & 0.527 & 15.163 & 0.499 &  &  & BCBBA \\
V226 & 0.48843 & RRab & 15.771 & 1.237 & 15.699 & 1.230 & 15.445 & 0.908 & 15.322 & 0.904 & 15.072 & 0.707 &  &  & BCBAB \\
V229 & 0.49762 & RRab & 15.883 & 1.663 & 15.881 & 1.573 & 15.593 & 1.159 & 15.565 & 0.750 & 15.166 & 0.790 &  &  & BCCBB \\
V234 & 0.50802 & RRab & 16.110 & 1.382 & 15.937 & 1.127 & 15.614 & 0.923 & 15.352 & 0.648 & 15.295 & 0.618 &  &  & BCCCB \\
V235 & 0.75984 & RRab & 15.790 & 0.601 & 15.844 & 0.548 & 15.447 & 0.477 & 15.105 & 0.320 & 14.856 & 0.278 & OoII &  & AAABA \\
V239 & 0.50398 & RRab & 15.930 & 1.022 & 15.971 & 1.292 & 15.654 & 0.915 & 15.523 & 0.940 & 15.203 & 0.763 &  & Bl & CBBBA \\
V240 & 0.27601 & RRc & 15.548 & 0.565 & 15.565 & 0.610 & 15.252 & 0.528 & 14.996 & 0.578 & 14.768 & 0.365 &  &  & CBBBB \\
V241 & 0.59617 & RRab & 15.805 & 1.291 & 15.818 & 1.457 & 15.503 & 1.154 & 15.330 & 0.879 & 15.033 & 0.844 &  &  & ABAAA \\
V242 & 0.59650 & RRab & 15.602 & 0.846 & 15.818 & 0.731 & 15.451 & 0.574 & 15.310 & 0.377 & 14.955 & 0.389 &  &  & ABAAA \\
V243 & 0.63462 & RRab & 15.778 & 0.877 & 15.879 & 0.673 & 15.482 & 0.554 & 15.225 & 0.536 & 14.861 & 0.373 &  & Bl & CAABA \\
V244 & 0.53784 & RRab & 15.766 & 1.215 & 15.839 & 1.301 & 15.553 & 1.090 & 15.347 & 1.076 & 15.200 & 0.832 &  &  & BCCAA \\
V245 & 0.28403 & RRc & 15.707 & 0.765 & 15.764 & 0.825 & 15.492 & 0.715 & 15.476 & 0.522 & 15.188 & 0.495 &  &  & CCBCB \\
V246 & 0.33914 & RRc & 15.705 & 0.770 & 15.762 & 0.830 & 15.496 & 0.719 & 15.309 & 0.525 & 15.095 & 0.498 &  &  & CCCBB \\
V247 & 0.60536 & RRab & 15.921 & 0.893 & 16.077 & 0.889 & 15.671 & 0.769 & 15.429 & 0.651 & 15.052 & 0.497 &  &  & CBBAA \\
V248 & 0.50979 & RRab & 15.730 & 0.996 & 15.859 & 1.001 & 15.589 & 0.813 & 15.426 & 0.554 & 15.030 & 0.541 &  &  & CCCBB \\
V249 & 0.53300 & RRab & 15.400 & 1.206 & 15.406 & 0.936 & 15.086 & 0.722 & 14.777 & 0.500 & 14.612 & 0.475 &  &  & BBBAA \\
V250n & 0.57438 & RRab & 16.023 & 1.014 & 16.064 & 1.160 & 15.710 & 0.950 & 15.421 & 1.047 & 15.120 & 0.574 &  &  & BBBAA \\
V250s & 0.59242 & RRab & 15.638 & 0.838 & 15.847 & 0.964 & 15.462 & 0.791 & 15.334 & 0.527 & 15.012 & 0.530 &  &  & BBBAA \\
V251 & 0.35392 & RRd & 15.260 & 0.632 & 15.300 & 0.682 & 15.112 & 0.836 & 14.976 & 0.431 & 14.861 & 0.409 &  &  & CCCBB \\
V252 & 0.30350 & RRd & 15.804 & 0.708 & 15.718 & 0.764 & 15.467 & 0.661 & 15.475 & 0.483 & 15.196 & 0.458 &  &  & CCBCB \\
V253 & 0.33262 & RRc & 15.393 & 0.677 & 15.518 & 0.730 & 15.281 & 0.633 & 15.120 & 0.473 & 14.913 & 0.438 &  &  & CBBAB \\
V254 & 0.60564 & RRab & 15.680 & 0.930 & 15.796 & 0.992 & 15.396 & 0.748 & 15.425 & 0.555 & 15.010 & 0.542 &  &  & CCCBC \\
V255 & 0.57271 & RRab & 15.794 & 0.752 & 15.860 & 0.833 & 15.440 & 0.595 & 15.148 & 0.418 & 14.864 & 0.392 &  & Bl & ABBAA \\
V256 & 0.31805 & RRc & 15.894 & 0.937 & 15.857 & 1.011 & 15.644 & 0.876 & 15.456 & 0.639 & 15.295 & 0.606 &  &  & CCCAB \\
V257 & 0.60206 & RRab & 15.698 & 0.818 & 15.768 & 0.886 & 15.425 & 0.705 & 15.300 & 0.751 & 14.916 & 0.426 &  &  & AAAAA \\
V258 & 0.71340 & RRab & 15.896 & 0.632 & 15.971 & 0.649 & 15.584 & 0.500 & 15.334 & 0.439 & 15.001 & 0.321 &  &  & BAAAA \\
V259 & 0.33352 & RRc & 15.481 & 0.399 & 15.501 & 0.431 & 15.080 & 0.373 & 14.815 & 0.272 & 14.467 & 0.258 &  &  & CBBBB \\
V261 & 0.44467 & RRc & 15.146 & 0.988 & 15.188 & 1.065 & 14.875 & 0.923 & 14.631 & 0.674 & 14.538 & 0.639 &  &  & CCCBB \\
V262 & 0.65505 & RRab & 15.664 & 0.527 & 15.880 & 0.569 & 15.479 & 0.467 & 15.439 & 0.294 & 15.015 & 0.261 &  &  & CCBAB \\
V264 & 0.35647 & RRc & 15.700 & 0.879 & 15.647 & 0.948 & 15.287 & 0.821 & 15.228 & 0.600 & 14.946 & 0.568 &  &  & CCCBB \\
V266 & 0.34244 & RRc & 15.630 & 0.562 & 15.710 & 0.606 & 15.411 & 0.525 & 15.234 & 0.575 & 14.967 & 0.358 &  &  & BBBAA \\
V269 & 0.35570 & RRc & 15.212 & 0.625 & 15.329 & 0.674 & 15.062 & 0.553 & 14.988 & 0.640 & 14.807 & 0.404 &  &  & CCCBB \\
V270n & 0.62586 & RRab & 15.740 & 0.653 & 15.814 & 0.799 & 15.457 & 0.659 & 15.254 & 0.563 & 14.930 & 0.386 &  &  & CBBAA \\
V270s & 0.69019 & RRab & 15.041 & 1.059 & 15.088 & 1.195 & 14.873 & 0.861 & 14.558 & 0.624 & 14.514 & 0.620 &  &  & CCBCB \\
V271 & 0.63280 & RRab & 16.084 & 0.817 & 16.088 & 0.807 & 15.674 & 0.594 & 15.403 & 0.340 & 15.069 & 0.367 &  &  & ABBAA \\
V290 & 0.24041 & RRd & 15.881 & 0.115 & 15.851 & 0.124 & 15.674 & 0.107 & 15.547 & 0.078 & 15.374 & 0.074 &  &  & BBBBA \\
V292 & 0.29654 & RRc & 15.785 & 0.472 & 15.778 & 0.509 & 15.603 & 0.441 & 15.501 & 0.322 & 15.331 & 0.305 &  &  & CCCAB \\
\end{tabular}



==> tables/table_2_long.tex <==
\begin{tabular}{ccccccccccccccccc}
\hline
Star Id & Period & |$\Delta P|$ & Type & <U> & A$_{\rm U}$ & <B> & A$_{\rm B}$ & <V> & A$_{\rm V}$ & <R> & A$_{\rm R}$ & <I> & A$_{\rm I}$ & Oo Type & Blazhko & QF \\
 & days & days &  & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ &  & & (UBVRI) \\
\hline
V1 & 0.52059 & 0.00001 & RRab & 15.470 & 0.635 & 16.221 & 0.694 & 15.824 & 0.568 & 15.525 & 0.441 & 15.266 & 0.356 & OoI & -- & CCBCB \\
V3 & 0.55820 & 0.00000 & RRab & 15.738 & 1.478 & 15.969 & 1.346 & 15.606 & 0.974 & 15.289 & 0.733 & 15.117 & 0.743 & OoII & Bl & AAACA \\
V4n & 0.58504 & 0.00004 & RRab & 15.074 & 0.808 & 15.114 & 0.932 & 14.754 & 0.763 & 14.430 & 0.595 & 14.205 & 0.487 & -- & -- & ABACA \\
V5 & 0.50583 & 0.00013 & RRab & 15.990 & 1.008 & 16.028 & 1.366 & 15.691 & 1.053 & 15.507 & 0.580 & 15.216 & 0.781 & OoI & Bl & AAACA \\
V6 & 0.51434 & 0.00004 & RRab & 16.012 & 1.419 & 16.045 & 1.268 & 15.693 & 1.130 & 15.498 & 0.715 & 15.243 & 0.813 & OoI & -- & ABACA \\
V7 & 0.49742 & 0.00002 & RRab & 15.679 & 0.794 & 15.678 & 0.881 & 15.394 & 0.606 & 15.212 & 0.495 & 15.163 & 0.499 & OoI & Bl & CCCCB \\
\vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
% V8 & 0.63672 & 0.00002 & RRab & 15.684 & 0.648 & 15.735 & 0.851 & 15.273 & 0.585 & 14.913 & 0.401 & 14.566 & 0.236 & -- & Bl & AAACA \\
% V9 & 0.55666 & 0.01506 & RRab & 16.272 & 0.969 & 15.928 & 1.291 & 15.643 & 1.019 & 15.601 & 0.502 & 15.181 & 0.783 & OoI & -- & BBBCA \\
% V10 & 0.56955 & 0.00005 & RRab & 15.975 & 1.103 & 16.051 & 1.106 & 15.719 & 0.748 & 15.402 & 0.593 & 15.153 & 0.512 & OoI & Bl & AAACA \\
% V11 & 0.50789 & 0.00001 & RRab & 15.395 & 1.119 & 16.032 & 1.577 & 15.712 & 1.191 & 15.450 & 1.011 & 15.224 & 0.831 & OoI & -- & CAACA \\
% V12 & 0.32557 & 0.00767 & RRc & 15.896 & 0.501 & 15.871 & 0.540 & 15.633 & 0.468 & 15.597 & 0.342 & 15.306 & 0.324 & -- & -- & BAACA \\
% V13 & 0.32350 & 0.02720 & RRd & 16.109 & 0.787 & 16.001 & 0.849 & 15.644 & 0.735 & 15.570 & 0.537 & 15.232 & 0.509 & -- & Bl & BBBCA \\
% V14 & 0.63590 & 0.00000 & RRab & 15.910 & 1.315 & 15.901 & 1.278 & 15.550 & 1.004 & 15.169 & 0.882 & 15.054 & 0.556 & OoII & Bl & AAACA \\
% V15 & 0.53009 & 0.00001 & RRab & 16.097 & 0.919 & 16.063 & 1.129 & 15.766 & 0.851 & 15.447 & 0.922 & 15.182 & 0.716 & OoI & -- & AAACA \\
% V16 & 0.51149 & 0.00001 & RRab & 16.054 & 1.465 & 16.103 & 1.460 & 15.766 & 1.134 & 15.546 & 1.008 & 15.270 & 0.827 & OoI & -- & AAACA \\
% V17 & 0.57616 & 0.00004 & RRab & 16.014 & 0.833 & 16.028 & 0.878 & 15.699 & 0.717 & 15.437 & 0.460 & 15.166 & 0.425 & OoI & Bl & AAACA \\
% V18 & 0.51645 & 0.00005 & RRab & 16.089 & 1.429 & 16.168 & 1.059 & 15.816 & 0.911 & 15.499 & 0.888 & 15.310 & 0.567 & OoI & -- & BAACA \\
% V19 & 0.63197 & 0.00003 & RRab & 16.081 & 0.653 & 16.107 & 0.579 & 15.722 & 0.435 & 15.442 & 0.387 & 15.156 & 0.288 & OoI & -- & AAACA \\
% V20 & 0.49752 & 0.00622 & RRab & 15.805 & 1.131 & 15.979 & 1.228 & 15.558 & 1.308 & 15.460 & 0.651 & 15.130 & 0.602 & OoI & Bl & CBBCA \\
% V21 & 0.51367 & 0.00213 & RRab & 16.026 & 0.934 & 16.158 & 1.180 & 15.776 & 0.875 & 15.620 & 0.493 & 15.203 & 0.452 & OoI & -- & AAACA \\
% V22 & 0.48141 & 0.00001 & RRab & 15.839 & 1.160 & 16.069 & 1.331 & 15.695 & 1.323 & 15.562 & 0.626 & 15.264 & 0.617 & OoI & Bl & AAACA \\
% V23 & 0.59538 & 0.00002 & RRab & 15.865 & 0.961 & 16.055 & 0.944 & 15.681 & 0.763 & 15.291 & 0.550 & 15.143 & 0.460 & OoI & Bl & AAACA \\
% V24 & 0.66340 & 0.00000 & RRab & 15.908 & 0.902 & 15.928 & 1.090 & 15.560 & 0.825 & 15.213 & 0.434 & 15.027 & 0.431 & OoII & Bl & AAACA \\
% V25 & 0.48006 & 0.00004 & RRab & 16.010 & 1.426 & 16.157 & 1.312 & 15.713 & 1.116 & 15.532 & 1.050 & 15.264 & 0.683 & OoI & -- & BBACA \\
% V26 & 0.59774 & 0.00004 & RRab & 15.922 & 1.184 & 15.961 & 1.177 & 15.618 & 0.906 & 15.374 & 0.788 & 15.089 & 0.668 & OoII & -- & AAACA \\
% V27 & 0.57906 & 0.00004 & RRab & 15.964 & 1.066 & 16.018 & 1.102 & 15.661 & 0.840 & 15.401 & 0.781 & 15.145 & 0.568 & OoI & -- & AAACA \\
% V28 & 0.47064 & 0.00004 & RRab & 15.934 & 1.223 & 15.960 & 1.378 & 15.690 & 1.053 & 15.511 & 0.793 & 15.247 & 0.640 & OoI & Bl & AAACA \\
% V29 & 0.47178 & 0.00178 & RRab & 15.773 & 1.060 & 15.895 & 1.171 & 15.576 & 0.970 & 15.405 & 0.649 & 15.193 & 0.653 & -- & -- & CCBCA \\
% V30 & 0.51209 & 0.00001 & RRab & 16.199 & 1.018 & 15.978 & 1.254 & 15.633 & 1.018 & 15.421 & 0.846 & 15.171 & 0.696 & -- & -- & AAACA \\
% V31 & 0.58073 & 0.00003 & RRab & 15.830 & 1.410 & 15.890 & 1.377 & 15.570 & 1.140 & 15.163 & 0.805 & 15.085 & 0.710 & OoII & -- & BAACA \\
% V32 & 0.49535 & 0.00005 & RRab & 16.093 & 0.896 & 15.930 & 1.382 & 15.613 & 1.100 & 15.513 & 0.627 & 15.106 & 0.698 & OoI & -- & AAACA \\
% V33 & 0.52525 & 0.00005 & RRab & 15.832 & 1.080 & 15.994 & 1.138 & 15.671 & 0.932 & 15.552 & 0.652 & 15.174 & 0.610 & OoI & Bl & CBBCA \\
% V34 & 0.55910 & 0.00430 & RRab & 16.012 & 0.746 & 16.072 & 0.903 & 15.718 & 0.743 & 15.372 & 0.694 & 15.203 & 0.440 & OoI & Bl & AAACA \\
% V35 & 0.52976 & 0.00074 & RRab & 15.919 & 1.208 & 16.040 & 1.354 & 15.723 & 1.110 & 15.465 & 0.730 & 15.242 & 0.633 & OoI & Bl & CAACA \\
% V36 & 0.54559 & 0.00001 & RRab & 15.931 & 1.402 & 16.075 & 1.285 & 15.729 & 1.011 & 15.341 & 0.556 & 15.206 & 0.752 & OoI & -- & AAACA \\
% V37 & 0.32664 & 0.00004 & RRc & 15.927 & 0.604 & 15.898 & 0.651 & 15.669 & 0.564 & 15.479 & 0.423 & 15.290 & 0.390 & -- & -- & AAACA \\
% V38 & 0.55801 & 0.00001 & RRab & 15.995 & 1.253 & 16.066 & 0.972 & 15.716 & 0.706 & 15.353 & 0.496 & 15.222 & 0.471 & OoI & Bl & AAACA \\
% V39 & 0.58707 & 0.00003 & RRab & 16.078 & 0.696 & 16.023 & 0.906 & 15.669 & 0.710 & 15.459 & 0.422 & 15.169 & 0.503 & OoI & Bl & AAACA \\
% V40 & 0.55154 & 0.00004 & RRab & 16.042 & 1.184 & 16.104 & 1.207 & 15.738 & 0.945 & 15.335 & 0.882 & 15.240 & 0.600 & OoI & -- & AAACA \\
% V41 & 0.48509 & 0.00081 & RRab & 16.014 & 1.435 & 16.010 & 1.511 & 15.626 & 1.067 & 15.476 & 0.862 & 15.275 & 0.586 & OoI & Bl & CBBCB \\
% V42 & 0.59008 & 0.00002 & RRab & 15.787 & 1.240 & 15.750 & 1.338 & 15.457 & 1.009 & 15.432 & 0.595 & 15.059 & 0.765 & OoII & -- & BBACA \\
% V43 & 0.54052 & 0.00002 & RRab & 16.022 & 1.397 & 16.032 & 1.337 & 15.711 & 1.050 & 15.458 & 0.823 & 15.189 & 0.674 & -- & Bl & AAACA \\
% V44 & 0.36810 & 0.03704 & RRd & 15.775 & 0.821 & 16.051 & 0.885 & 15.606 & 0.767 & 15.113 & 0.560 & 15.271 & 0.531 & -- & Bl & BBBCB \\
% V45 & 0.53691 & 0.00001 & RRab & 16.248 & 0.969 & 16.229 & 1.036 & 15.784 & 0.849 & 15.570 & 0.725 & 15.291 & 0.557 & OoI & Bl & CAACA \\
% V46 & 0.61339 & 0.00001 & RRab & 16.036 & 0.758 & 16.108 & 0.688 & 15.712 & 0.500 & 15.425 & 0.374 & 15.149 & 0.361 & OoI & -- & AAACA \\
% V47 & 0.57257 & 0.03167 & RRab & 15.927 & 0.890 & 15.923 & 0.952 & 15.594 & 0.780 & 15.506 & 0.448 & 15.192 & 0.531 & OoI & Bl & BBBCB \\
% V48 & 0.62784 & 0.00004 & RRab & 15.893 & 0.597 & 15.935 & 0.685 & 15.544 & 0.506 & 15.245 & 0.392 & 14.959 & 0.378 & OoI? & Bl & AAACA \\
% V49 & 0.54821 & 0.00001 & RRab & 15.938 & 1.113 & 15.920 & 1.105 & 15.544 & 0.944 & 15.409 & 0.652 & 15.170 & 0.628 & OoI & Bl & ACBCA \\
% V50 & 0.51310 & 0.00030 & RRab & 16.096 & 1.300 & 16.063 & 1.268 & 15.672 & 1.117 & 15.513 & 0.767 & 15.257 & 0.590 & OoI & Bl & AAACA \\
% V51 & 0.58397 & 0.00003 & RRab & 16.001 & 0.940 & 16.042 & 1.035 & 15.691 & 0.811 & 15.391 & 0.592 & 15.150 & 0.585 & OoI & -- & AAACA \\
% V52 & 0.51624 & 0.00004 & RRab & 16.188 & 1.204 & 15.965 & 1.249 & 15.674 & 0.899 & 15.459 & 0.631 & 15.247 & 0.802 & OoI & Bl & BBBCA \\
% V53 & 0.50488 & 0.00002 & RRab & 16.298 & 0.435 & 16.358 & 0.469 & 15.994 & 0.396 & 15.656 & 0.249 & 15.286 & 0.248 & OoI & -- & BCBCB \\
% V54 & 0.50620 & 0.00010 & RRab & 16.056 & 0.836 & 16.170 & 0.942 & 15.779 & 0.727 & 15.523 & 0.712 & 15.239 & 0.420 & OoI & Bl & BBBCA \\
% V55 & 0.52983 & 0.00003 & RRab & 16.150 & 1.209 & 16.013 & 1.094 & 15.683 & 0.895 & 15.447 & 0.774 & 15.228 & 0.717 & OoI & -- & AAACA \\
% V56 & 0.32960 & 0.00000 & RRc & 15.874 & 0.553 & 15.926 & 0.579 & 15.648 & 0.468 & 15.469 & 0.404 & 15.278 & 0.304 & -- & -- & AAACA \\
% V57 & 0.51218 & 0.00002 & RRab & 16.143 & 1.099 & 16.116 & 1.214 & 15.753 & 0.968 & 15.564 & 0.779 & 15.184 & 0.583 & OoI & -- & BAACA \\
% V58 & 0.51705 & 0.00005 & RRab & 15.999 & 1.600 & 15.858 & 1.455 & 15.619 & 1.151 & 15.409 & 0.685 & 15.190 & 0.827 & OoI & -- & AAACA \\
% V59 & 0.58883 & 0.00003 & RRab & 16.062 & 0.970 & 16.076 & 0.927 & 15.693 & 0.744 & 15.459 & 0.543 & 15.182 & 0.466 & OoI & Bl & AAACA \\
% V60 & 0.70773 & 0.00003 & RRab & 15.956 & 0.844 & 15.949 & 0.845 & 15.566 & 0.646 & 15.344 & 0.603 & 15.012 & 0.415 & OoII & -- & AAACA \\
% V61 & 0.52089 & 0.00001 & RRab & 16.051 & 1.097 & 16.119 & 1.004 & 15.738 & 0.732 & 15.589 & 0.434 & 15.196 & 0.571 & -- & -- & AAACA \\
% V62 & 0.65240 & 0.00000 & RRab & 16.002 & 0.675 & 16.045 & 0.668 & 15.645 & 0.490 & 15.384 & 0.515 & 15.079 & 0.323 & OoI & Bl & AAACA \\
% V63 & 0.57040 & 0.00001 & RRab & 16.025 & 1.215 & 16.076 & 1.232 & 15.722 & 0.889 & 15.523 & 0.580 & 15.189 & 0.586 & OoI & Bl & AAACA \\
% V64 & 0.60546 & 0.00004 & RRab & 16.066 & 0.841 & 16.101 & 0.945 & 15.714 & 0.711 & 15.461 & 0.607 & 15.158 & 0.444 & OoI & -- & AAACA \\
% V65 & 0.66716 & 0.00114 & RRab & 16.057 & 0.999 & 15.959 & 1.156 & 15.582 & 0.946 & 15.377 & 0.527 & 15.010 & 0.592 & OoII & -- & BAACA \\
% V66 & 0.62019 & 0.00001 & RRab & 16.010 & 0.705 & 16.060 & 0.784 & 15.657 & 0.615 & 15.412 & 0.461 & 15.125 & 0.366 & OoI & Bl & ABACA \\
% V67 & 0.56833 & 0.00003 & RRab & 16.041 & 0.704 & 16.113 & 0.854 & 15.720 & 0.746 & 15.479 & 0.617 & 15.193 & 0.476 & OoI & Bl & AAACA \\
% V68 & 0.36053 & 0.00453 & RRd & 15.932 & 0.675 & 15.823 & 0.728 & 15.528 & 0.630 & 15.411 & 0.460 & 15.222 & 0.436 & -- & -- & BBBCA \\
% V69 & 0.56662 & 0.00002 & RRab & 16.113 & 1.087 & 16.089 & 1.157 & 15.730 & 0.899 & 15.448 & 0.698 & 15.193 & 0.545 & OoI & -- & AAACA \\
% V70 & 0.48606 & 0.00034 & RRc & 15.576 & 0.360 & 15.675 & 0.425 & 15.368 & 0.340 & 15.168 & 0.253 & 14.921 & 0.232 & -- & Bl & AAACA \\
% V71 & 0.54905 & 0.00005 & RRab & 15.958 & 1.132 & 16.083 & 1.166 & 15.725 & 0.905 & 15.511 & 0.705 & 15.181 & 0.531 & OoI & Bl & AAACA \\
% V72 & 0.45608 & 0.00002 & RRab & 15.839 & 1.487 & 15.945 & 1.461 & 15.716 & 1.190 & 15.293 & 0.882 & 15.332 & 0.726 & OoI & -- & BAACA \\
% V73 & 0.67348 & 0.00012 & RRab & 16.001 & 0.430 & 16.073 & 0.350 & 15.671 & 0.272 & 15.348 & 0.227 & 15.074 & 0.155 & OoI & Bl & AAACA \\
% V74 & 0.49216 & 0.00004 & RRab & 16.070 & 1.528 & 16.060 & 1.633 & 15.671 & 1.350 & 15.570 & 0.850 & 15.285 & 0.713 & OoI & -- & ABACB \\
% V75 & 0.31408 & 0.00002 & RRc & 15.913 & 0.554 & 15.936 & 0.578 & 15.686 & 0.489 & 15.518 & 0.357 & 15.303 & 0.338 & -- & -- & AAACA \\
% V76 & 0.50176 & 0.00004 & RRab & 15.938 & 1.591 & 16.049 & 1.518 & 15.720 & 1.203 & 15.331 & 0.582 & 15.266 & 0.724 & OoI & -- & AAACA \\
% V77 & 0.45935 & 0.00005 & RRab & 16.397 & 0.855 & 15.999 & 1.133 & 15.805 & 1.015 & 15.783 & 0.586 & 15.446 & 0.559 & OoI & Bl & CCCCC \\
% V78 & 0.61191 & 0.00001 & RRab & 15.855 & 0.970 & 16.017 & 0.812 & 15.667 & 0.607 & 15.413 & 0.395 & 15.086 & 0.381 & OoII? & Bl & AAACA \\
% V79 & 0.48326 & 0.00004 & RRab & 16.161 & 0.893 & 16.187 & 0.973 & 15.910 & 0.790 & 15.513 & 0.469 & 15.337 & 0.466 & OoI & Bl & BBBCA \\
% V80 & 0.52906 & 0.00934 & RRab & 16.022 & 0.809 & 16.254 & 0.899 & 15.739 & 0.852 & 15.401 & 0.572 & 15.293 & 0.521 & OoI & Bl & BCBCA \\
% V81 & 0.52912 & 0.00002 & RRab & 15.812 & 1.393 & 16.132 & 1.199 & 15.706 & 1.083 & 15.450 & 0.675 & 15.216 & 0.730 & OoI & -- & AAACA \\
% V82 & 0.52454 & 0.00004 & RRab & 16.035 & 1.438 & 16.078 & 1.355 & 15.744 & 1.061 & 15.475 & 0.948 & 15.228 & 0.719 & OoI & -- & AAACA \\
% V83 & 0.50127 & 0.00003 & RRab & 16.092 & 0.979 & 16.141 & 1.320 & 15.766 & 0.952 & 15.692 & 0.512 & 15.287 & 0.859 & OoI & -- & AAACA \\
% V84 & 0.59573 & 0.00003 & RRab & 15.985 & 1.018 & 16.064 & 0.933 & 15.704 & 0.698 & 15.394 & 0.633 & 15.145 & 0.486 & OoI & -- & AAACA \\
% V85 & 0.35581 & 0.00001 & RRc & 15.835 & 0.538 & 15.740 & 0.546 & 15.512 & 0.430 & 15.360 & 0.314 & 15.154 & 0.297 & -- & -- & AAACA \\
% V86 & 0.29266 & 0.00004 & RRc & 15.948 & 0.484 & 15.899 & 0.645 & 15.695 & 0.498 & 15.490 & 0.330 & 15.327 & 0.313 & -- & -- & AAACA \\
% V87 & 0.35748 & 0.00002 & RRd & 15.846 & 0.510 & 15.871 & 0.550 & 15.593 & 0.476 & 15.299 & 0.348 & 15.146 & 0.329 & -- & -- & AAACA \\
% V88 & 0.29875 & 0.00005 & RRc & 15.940 & 0.703 & 15.922 & 0.758 & 15.701 & 0.657 & 15.415 & 0.480 & 15.370 & 0.454 & -- & -- & AAACA \\
% V89 & 0.54848 & 0.00002 & RRab & 16.042 & 1.107 & 16.004 & 1.309 & 15.663 & 0.999 & 15.388 & 0.743 & 15.139 & 0.624 & OoI & -- & AAACA \\
% V90 & 0.51703 & 0.00003 & RRab & 16.000 & 1.370 & 16.078 & 1.356 & 15.782 & 1.055 & 15.543 & 0.850 & 15.234 & 0.751 & OoI & -- & AAACA \\
% V91 & 0.53011 & 0.00071 & RRab & 15.859 & 1.018 & 16.066 & 1.168 & 15.702 & 0.804 & 15.409 & 0.770 & 15.202 & 0.479 & OoI & Bl & AAACA \\
% V92 & 0.50355 & 0.00005 & RRab & 15.964 & 0.874 & 16.113 & 0.814 & 15.783 & 0.677 & 15.481 & 0.448 & 15.415 & 0.447 & OoI & Bl & CCCCB \\
% V93 & 0.60230 & 0.00000 & RRab & 15.935 & 0.830 & 16.108 & 0.896 & 15.718 & 0.667 & 15.529 & 0.644 & 15.183 & 0.502 & OoI & -- & AAABA \\
% V94 & 0.52370 & 0.00000 & RRab & 16.335 & 0.899 & 15.948 & 1.042 & 15.720 & 0.848 & 15.493 & 0.546 & 15.298 & 0.541 & OoI & -- & CBBCA \\
% V96 & 0.49941 & 0.00001 & RRab & 15.624 & 0.769 & 16.234 & 0.985 & 15.858 & 0.813 & 15.529 & 0.705 & 15.377 & 0.699 & OoI & -- & BAACA \\
% V97 & 0.33493 & 0.00003 & RRc & 16.059 & 0.392 & 15.976 & 0.508 & 15.710 & 0.409 & 15.518 & 0.343 & 15.311 & 0.254 & -- & -- & AAACA \\
% V99 & 0.35543 & 0.00567 & RRd & 15.760 & 0.526 & 15.913 & 0.567 & 15.665 & 0.491 & 15.375 & 0.391 & 15.158 & 0.340 & -- & Bl & BAACA \\
% V100 & 0.61881 & 0.00001 & RRab & 15.988 & 0.657 & 16.177 & 0.583 & 15.744 & 0.502 & 15.452 & 0.489 & 15.101 & 0.273 & OoI & -- & AAACA \\
% V101 & 0.64389 & 0.00001 & RRab & 16.013 & 0.645 & 16.065 & 0.652 & 15.669 & 0.537 & 15.370 & 0.364 & 15.110 & 0.359 & OoI & Bl & AAACA \\
% V104 & 0.56993 & 0.00003 & RRab & 15.832 & 1.424 & 15.917 & 1.421 & 15.610 & 1.127 & 15.362 & 0.852 & 15.110 & 0.706 & OoII & Bl & AAACA \\
% V105 & 0.28775 & 0.00005 & RRc & 15.866 & 0.408 & 15.819 & 0.440 & 15.619 & 0.381 & 15.440 & 0.287 & 15.334 & 0.264 & -- & -- & AAACA \\
% V106 & 0.53725 & 0.00985 & RRab & 16.016 & 0.745 & 16.040 & 0.876 & 15.695 & 0.661 & 15.492 & 0.379 & 15.234 & 0.444 & OoI & Bl & BAACA \\
% V107 & 0.30903 & 0.00003 & RRc & 16.089 & 0.490 & 15.874 & 0.528 & 15.664 & 0.458 & 15.312 & 0.334 & 15.342 & 0.317 & -- & -- & BAACA \\
% V108 & 0.51961 & 0.00001 & RRab & 16.080 & 1.414 & 16.084 & 1.376 & 15.764 & 1.079 & 15.546 & 0.646 & 15.273 & 0.745 & OoI & -- & AAACA \\
% V109 & 0.53392 & 0.00002 & RRab & 16.109 & 1.270 & 16.064 & 1.422 & 15.706 & 1.057 & 15.295 & 0.752 & 15.202 & 0.754 & OoI & -- & AAACA \\
% V110 & 0.53546 & 0.00004 & RRab & 16.034 & 0.970 & 16.009 & 1.127 & 15.671 & 0.924 & 15.375 & 0.688 & 15.168 & 0.617 & OoI & Bl & AAACB \\
% V111 & 0.51019 & 0.00001 & RRab & 15.866 & 1.108 & 16.070 & 1.065 & 15.738 & 0.923 & 15.345 & 0.566 & 15.246 & 0.557 & OoI & Bl & AAACA \\
% V113 & 0.51300 & 0.01121 & RRab & 16.200 & 1.095 & 15.981 & 1.497 & 15.674 & 1.196 & 15.502 & 0.574 & 15.153 & 0.654 & OoI & -- & BBACA \\
% V114 & 0.59772 & 0.00002 & RRab & 15.981 & 1.012 & 16.092 & 0.972 & 15.693 & 0.780 & 15.467 & 0.539 & 15.154 & 0.456 & OoI & Bl & AAABA \\
% V115 & 0.51335 & 0.00005 & RRab & 15.821 & 1.352 & 16.039 & 1.527 & 15.710 & 1.188 & 15.387 & 0.736 & 15.236 & 0.742 & OoI & -- & AAACA \\
% V116 & 0.51481 & 0.00001 & RRab & 16.074 & 1.338 & 15.999 & 1.326 & 15.696 & 1.040 & 15.499 & 0.807 & 15.274 & 0.741 & OoI & -- & AAACA \\
% V117 & 0.60054 & 0.00004 & RRab & 16.076 & 1.100 & 15.994 & 1.209 & 15.649 & 0.836 & 15.427 & 0.675 & 15.125 & 0.583 & OoI & Bl & AAACA \\
% V118 & 0.49940 & 0.00287 & RRab & 16.476 & 1.150 & 15.968 & 1.538 & 15.737 & 1.212 & 15.728 & 0.668 & 15.278 & 0.809 & -- & -- & BBACA \\
% V119 & 0.51835 & 0.00065 & RRab & 16.177 & 1.106 & 15.910 & 1.269 & 15.673 & 0.969 & 15.331 & 0.566 & 15.242 & 0.666 & OoI & Bl & CAACA \\
% V120 & 0.64014 & 0.00004 & RRab & 16.048 & 0.547 & 16.091 & 0.583 & 15.699 & 0.404 & 15.399 & 0.241 & 15.128 & 0.302 & OoI & -- & AAACA \\
% V121 & 0.53521 & 0.00001 & RRab & 16.022 & 1.320 & 16.039 & 1.242 & 15.708 & 0.928 & 15.466 & 0.640 & 15.167 & 0.656 & OoI & Bl & AAACA \\
% V122 & 0.51093 & 0.00507 & RRab & 16.196 & 1.048 & 16.114 & 1.301 & 15.711 & 1.166 & 15.657 & 0.922 & 15.255 & 0.661 & -- & -- & BBBCA \\
% V123 & 0.54548 & 0.00002 & RRab & 16.040 & 1.267 & 15.981 & 1.306 & 15.659 & 1.046 & 15.434 & 0.610 & 15.194 & 0.719 & OoI & -- & AAACA \\
% V124 & 0.75244 & 0.00004 & RRab & 15.920 & 0.517 & 15.967 & 0.459 & 15.566 & 0.356 & 15.268 & 0.290 & 14.982 & 0.229 & OoII & -- & AAACA \\
% V125 & 0.34982 & 0.00002 & RRd & 15.900 & 0.486 & 15.963 & 0.496 & 15.707 & 0.368 & 15.487 & 0.288 & 15.225 & 0.255 & -- & -- & AAACA \\
% V126 & 0.34840 & 0.00000 & RRc & 15.951 & 0.428 & 15.972 & 0.462 & 15.686 & 0.400 & 15.440 & 0.193 & 15.244 & 0.277 & -- & Bl & AAACA \\
% V128 & 0.29204 & 0.00004 & RRc & 15.880 & 0.540 & 15.878 & 0.651 & 15.654 & 0.535 & 15.551 & 0.363 & 15.311 & 0.344 & -- & -- & AAACA \\
% V130 & 0.55904 & 0.00706 & RRab & 15.851 & 0.829 & 15.975 & 0.861 & 15.603 & 0.710 & 15.384 & 0.474 & 15.107 & 0.421 & OoI & Bl & BAACA \\
% V131 & 0.29769 & 0.00001 & RRc & 15.840 & 0.558 & 15.865 & 0.631 & 15.640 & 0.506 & 15.520 & 0.488 & 15.277 & 0.351 & -- & -- & AAACA \\
% V132 & 0.33986 & 0.00004 & RRc & 15.814 & 0.467 & 15.893 & 0.453 & 15.621 & 0.380 & 15.509 & 0.278 & 15.209 & 0.263 & -- & -- & AAACA \\
% V133 & 0.55073 & 0.00003 & RRab & 16.187 & 0.996 & 15.906 & 1.064 & 15.725 & 0.977 & 15.523 & 0.600 & 15.198 & 0.587 & OoI & Bl & ABACA \\
% V134 & 0.61806 & 0.00004 & RRab & 15.943 & 0.798 & 16.049 & 0.784 & 15.655 & 0.574 & 15.454 & 0.482 & 15.102 & 0.392 & -- & -- & AAACA \\
% V135 & 0.56839 & 0.00001 & RRab & 15.709 & 0.899 & 16.022 & 1.168 & 15.661 & 0.885 & 15.393 & 0.585 & 15.129 & 0.608 & OoI & Bl & AAACA \\
% V136 & 0.61718 & 0.00002 & RRab & 15.793 & 0.800 & 15.909 & 0.797 & 15.520 & 0.632 & 15.203 & 0.628 & 14.956 & 0.405 & -- & -- & AAACA \\
% V137 & 0.57515 & 0.00005 & RRab & 15.837 & 1.114 & 15.986 & 1.088 & 15.620 & 0.879 & 15.315 & 0.486 & 15.099 & 0.481 & OoI & -- & AAACA \\
% V139 & 0.55999 & 0.00001 & RRab & 15.784 & 1.408 & 15.849 & 1.347 & 15.484 & 1.098 & 15.217 & 1.036 & 15.044 & 0.822 & -- & -- & AAACA \\
% V140 & 0.33314 & 0.00004 & RRc & 15.698 & 0.475 & 15.731 & 0.529 & 15.499 & 0.418 & 15.264 & 0.352 & 15.132 & 0.272 & -- & Bl & AAACA \\
% V142 & 0.56863 & 0.00003 & RRab & 15.974 & 1.198 & 16.094 & 1.219 & 15.710 & 0.968 & 15.477 & 0.826 & 15.203 & 0.644 & OoI & -- & AAACA \\
% V143 & 0.59654 & 0.00004 & RRab & 15.473 & 0.980 & 15.895 & 0.848 & 15.435 & 0.703 & 15.202 & 0.481 & 14.809 & 0.503 & OoII & Bl & CBACA \\
% V144 & 0.59679 & 0.00001 & RRab & 15.946 & 0.583 & 15.994 & 0.618 & 15.601 & 0.506 & 15.281 & 0.346 & 15.058 & 0.344 & -- & -- & AAACA \\
% V145 & 0.51449 & 0.00001 & RRab & 15.627 & 0.998 & 15.755 & 1.116 & 15.408 & 0.841 & 15.045 & 0.533 & 14.875 & 0.576 & -- & -- & AAACA \\
% V146 & 0.50220 & 0.00000 & RRab & 15.754 & 1.079 & 15.972 & 1.178 & 15.659 & 0.915 & 15.579 & 0.894 & 15.192 & 0.669 & OoI & -- & BAACA \\
% V147 & 0.34648 & 0.00002 & RRc & 15.836 & 0.475 & 15.954 & 0.514 & 15.657 & 0.444 & 15.448 & 0.424 & 15.260 & 0.307 & -- & -- & AAACA \\
% V148 & 0.46727 & 0.00003 & RRab & 16.158 & 1.314 & 16.200 & 1.654 & 15.808 & 1.497 & 15.453 & 1.460 & 15.354 & 1.030 & -- & -- & CBBCB \\
% V149 & 0.54818 & 0.00002 & RRab & 16.099 & 0.952 & 15.931 & 1.298 & 15.622 & 0.971 & 15.381 & 0.595 & 15.140 & 0.520 & -- & Bl & AAACA \\
% V150 & 0.52392 & 0.00002 & RRab & 15.744 & 1.246 & 16.028 & 1.252 & 15.674 & 1.000 & 15.529 & 0.743 & 15.211 & 0.638 & OoI & Bl & AAACA \\
% V151 & 0.51682 & 0.00002 & RRab & 15.630 & 0.913 & 16.038 & 1.009 & 15.660 & 0.825 & 15.507 & 0.555 & 15.148 & 0.571 & -- & Bl & BBBCA \\
% V152 & 0.32613 & 0.00003 & RRc & 15.712 & 0.480 & 15.697 & 0.517 & 15.493 & 0.448 & 15.328 & 0.327 & 15.179 & 0.310 & -- & -- & AAACA \\
% V155 & 0.33232 & 0.00062 & RRc & 15.758 & 0.702 & 15.793 & 0.757 & 15.544 & 0.656 & 15.298 & 0.479 & 15.177 & 0.454 & -- & -- & BAACA \\
% V156 & 0.53199 & 0.00001 & RRab & 15.776 & 1.204 & 15.836 & 1.280 & 15.501 & 0.988 & 15.225 & 0.805 & 15.032 & 0.626 & -- & -- & AAACA \\
% V157 & 0.54284 & 0.00006 & RRab & 15.465 & 0.659 & 16.111 & 0.710 & 15.634 & 0.610 & 15.144 & 0.381 & 14.920 & 0.386 & -- & Bl & CCBCB \\
% V159 & 0.53380 & 0.00010 & RRab & 15.473 & 0.899 & 15.662 & 0.993 & 15.138 & 0.853 & 15.015 & 0.567 & 14.737 & 0.532 & -- & Bl & BCBCA \\
% V160 & 0.65732 & 0.00002 & RRab & 15.729 & 1.044 & 15.863 & 1.109 & 15.500 & 0.924 & 15.329 & 0.617 & 15.009 & 0.576 & -- & Bl & BAACA \\
% V161 & 0.52515 & 0.00135 & RRab & 15.853 & 1.096 & 15.858 & 1.314 & 15.525 & 1.002 & 15.131 & 0.653 & 14.948 & 0.639 & -- & Bl & CBBCB \\
% V165 & 0.48363 & 0.00003 & RRab & 16.014 & 1.260 & 15.790 & 1.503 & 15.452 & 1.325 & 15.516 & 0.747 & 15.139 & 0.720 & -- & Bl & ABBCA \\
% V166 & 0.32266 & 0.03404 & RRd & 16.140 & 0.716 & 15.960 & 0.772 & 15.693 & 0.669 & 15.494 & 0.488 & 15.262 & 0.463 & -- & Bl & BBACB \\
% V167 & 0.64396 & 0.00004 & RRab & 15.967 & 0.531 & 16.078 & 0.515 & 15.687 & 0.383 & 15.380 & 0.407 & 15.119 & 0.276 & OoI & Bl & AAACA \\
% V168 & 0.27594 & 0.00004 & RRc & 15.734 & 0.532 & 15.796 & 0.574 & 15.582 & 0.497 & 15.397 & 0.363 & 15.204 & 0.344 & -- & Bl & AAACA \\
% V170 & 0.43230 & 0.01235 & RRc & 15.506 & 0.475 & 15.480 & 0.513 & 15.259 & 0.444 & 15.145 & 0.324 & 14.855 & 0.307 & -- & -- & BBBCA \\
% V171 & 0.30506 & 0.00176 & RRc & 15.787 & 0.658 & 15.723 & 0.709 & 15.483 & 0.614 & 15.401 & 0.449 & 15.218 & 0.425 & -- & -- & CAACA \\
% V172 & 0.54229 & 0.00001 & RRab & 16.205 & 0.374 & 15.711 & 0.760 & 15.602 & 0.557 & 15.716 & 0.424 & 15.306 & 0.407 & -- & -- & BCCCB \\
% V173 & 0.60700 & 0.00001 & RRab & 15.598 & 1.242 & 15.797 & 1.411 & 15.356 & 1.104 & 15.244 & 1.129 & 14.959 & 0.734 & -- & -- & BBBCA \\
% V174 & 0.59130 & 0.01151 & RRab & 16.010 & 0.770 & 16.036 & 0.823 & 15.642 & 0.674 & 15.406 & 0.686 & 15.073 & 0.463 & -- & Bl & BCBCA \\
% V175 & 0.56970 & 0.00000 & RRab & 15.988 & 1.169 & 16.075 & 1.146 & 15.714 & 0.815 & 15.406 & 0.689 & 15.163 & 0.558 & -- & -- & AAACA \\
% V176 & 0.53962 & 0.00002 & RRab & 16.065 & 0.794 & 15.989 & 0.846 & 15.693 & 0.692 & 15.536 & 0.706 & 15.222 & 0.469 & -- & Bl & BAACA \\
% V177 & 0.34835 & 0.00005 & RRc & 15.732 & 0.582 & 15.728 & 0.581 & 15.509 & 0.459 & 15.350 & 0.353 & 15.140 & 0.318 & -- & -- & AAACA \\
% V178 & 0.26696 & 0.00004 & RRc & 15.847 & 0.396 & 15.862 & 0.427 & 15.680 & 0.370 & 15.563 & 0.270 & 15.380 & 0.256 & -- & -- & AAACA \\
% V180 & 0.60910 & 0.00000 & RRab & 15.772 & 0.681 & 16.007 & 0.732 & 15.587 & 0.627 & 15.314 & 0.420 & 15.023 & 0.405 & -- & -- & BAACB \\
% V181 & 0.66385 & 0.00005 & RRab & 15.699 & 0.859 & 15.886 & 0.905 & 15.478 & 0.743 & 15.037 & 0.753 & 14.863 & 0.490 & -- & -- & BAACB \\
% V184 & 0.53123 & 0.00003 & RRab & 15.867 & 1.142 & 15.913 & 1.289 & 15.619 & 1.019 & 15.489 & 0.690 & 15.179 & 0.701 & -- & Bl & BBACA \\
% V186 & 0.66325 & 0.00015 & RRab & 15.873 & 0.563 & 15.975 & 0.588 & 15.591 & 0.479 & 15.191 & 0.330 & 15.013 & 0.358 & -- & Bl & AAACA \\
% V187 & 0.58628 & 0.00002 & RRab & 15.951 & 1.199 & 16.030 & 1.065 & 15.643 & 0.761 & 15.411 & 0.658 & 15.152 & 0.539 & -- & -- & BAACB \\
% V188 & 0.26652 & 0.00002 & RRc & 15.880 & 0.429 & 15.902 & 0.463 & 15.693 & 0.401 & 15.604 & 0.293 & 15.392 & 0.278 & -- & -- & AAACA \\
% V189 & 0.61294 & 0.00004 & RRab & 15.782 & 1.012 & 15.946 & 0.901 & 15.503 & 0.737 & 15.311 & 0.601 & 14.919 & 0.409 & -- & -- & AAACA \\
% V190 & 0.52280 & 0.00000 & RRab & 15.947 & 1.356 & 16.013 & 1.396 & 15.673 & 1.082 & 15.277 & 0.892 & 15.196 & 0.688 & -- & -- & AAACA \\
% V191 & 0.51919 & 0.00001 & RRab & 15.815 & 1.356 & 16.033 & 1.457 & 15.678 & 1.266 & 15.615 & 0.742 & 15.257 & 0.654 & -- & Bl & BAACA \\
% V192 & 0.49740 & 0.00009 & RRab & 14.542 & 0.615 & 14.757 & 0.657 & 14.149 & 0.538 & 13.829 & 0.368 & 13.367 & 0.356 & -- & Bl & BBACA \\
% V193 & 0.74787 & 0.00003 & RRab & 15.361 & 1.015 & 15.498 & 1.037 & 15.129 & 0.892 & 14.897 & 0.893 & 14.637 & 0.645 & -- & -- & AAACA \\
% V194 & 0.48920 & 0.00001 & RRab & 15.396 & 1.142 & 15.567 & 1.181 & 15.091 & 0.844 & 14.808 & 0.959 & 14.543 & 0.615 & -- & -- & BBACB \\
% V195 & 0.64392 & 0.00018 & RRab & 15.845 & 0.902 & 15.877 & 1.031 & 15.568 & 0.603 & 15.287 & 0.551 & 14.997 & 0.555 & -- & Bl & CBBCA \\
% V197 & 0.49990 & 0.00001 & RRab & 16.113 & 1.238 & 16.086 & 1.443 & 15.718 & 1.175 & 15.194 & 0.719 & 15.275 & 0.717 & -- & -- & BAACA \\
% V200 & 0.36100 & 0.03456 & RRd & 15.393 & 0.821 & 15.820 & 0.885 & 15.500 & 0.913 & 15.256 & 0.560 & 14.985 & 0.531 & -- & -- & CBBCC \\
% V201 & 0.54053 & 0.00003 & RRab & 15.186 & 0.948 & 15.571 & 1.079 & 15.142 & 0.882 & 14.836 & 0.574 & 14.828 & 0.577 & -- & Bl & BBBCC \\
% V202 & 0.77357 & 0.00003 & RRab & 15.925 & 0.225 & 15.973 & 0.193 & 15.563 & 0.138 & 15.269 & 0.153 & 14.974 & 0.096 & OoII & -- & AAACA \\
% V203 & 0.28980 & 0.00001 & RRc & 15.838 & 0.189 & 15.758 & 0.204 & 15.599 & 0.177 & 15.428 & 0.129 & 15.299 & 0.122 & -- & Bl & AAACA \\
% V205 & 0.63690 & 0.00521 & RRab & 16.035 & 0.648 & 16.128 & 0.483 & 15.716 & 0.421 & -- & -- & 15.152 & 0.236 & OoI & -- & AAACA \\
% V207 & 0.34531 & 0.00001 & RRc & 15.698 & 0.609 & 15.816 & 0.657 & 15.526 & 0.569 & 15.264 & 0.433 & 15.079 & 0.394 & -- & -- & AAACA \\
% V208 & 0.33839 & 0.00001 & RRc & 15.769 & 0.429 & 15.801 & 0.476 & 15.511 & 0.401 & 15.254 & 0.293 & 15.026 & 0.278 & -- & -- & AAACA \\
% V209 & 0.34828 & 0.00002 & RRc & 15.818 & 0.520 & 15.799 & 0.561 & 15.556 & 0.486 & 15.373 & 0.427 & 15.181 & 0.336 & -- & -- & AAACA \\
% V210 & 0.35295 & 0.00005 & RRc & 15.883 & 0.581 & 15.919 & 0.627 & 15.668 & 0.543 & 15.438 & 0.460 & 15.243 & 0.376 & -- & -- & AAACB \\
% V211 & 0.55820 & 0.00000 & RRab & 15.908 & 1.182 & 16.125 & 1.106 & 15.721 & 0.943 & 15.256 & 0.605 & 15.295 & 0.624 & -- & Bl & BABCB \\
% V212 & 0.54220 & 0.00000 & RRab & 15.827 & 1.069 & 15.915 & 1.177 & 15.586 & 0.966 & 15.389 & 0.732 & 15.113 & 0.558 & -- & Bl & AAACA \\
% V213 & 0.30000 & 0.00000 & RRc & 15.615 & 0.487 & 15.621 & 0.526 & 15.347 & 0.455 & 15.171 & 0.333 & 14.966 & 0.315 & -- & -- & BAACA \\
% V214 & 0.53951 & 0.00001 & RRab & 15.839 & 1.430 & 16.016 & 1.253 & 15.649 & 1.026 & 15.412 & 0.671 & 15.128 & 0.666 & -- & Bl & AAACA \\
% V215 & 0.52870 & 0.00000 & RRab & 15.594 & 0.914 & 15.708 & 0.991 & 15.412 & 0.812 & 15.244 & 0.533 & 15.085 & 0.536 & -- & -- & BBBCB \\
% V216 & 0.34648 & 0.00002 & RRc & 15.745 & 0.533 & 15.828 & 0.575 & 15.560 & 0.498 & 15.380 & 0.363 & 15.161 & 0.344 & -- & -- & AAACA \\
% V217 & 0.52836 & 0.00004 & RRab & 15.476 & 1.406 & 15.728 & 1.194 & 15.387 & 0.982 & 15.264 & 0.942 & 14.948 & 0.679 & -- & -- & AAACB \\
% V218 & 0.54487 & 0.00003 & RRab & 15.920 & 0.982 & 15.992 & 1.020 & 15.630 & 0.843 & 15.414 & 0.510 & 15.067 & 0.562 & OoI & Bl & AAACA \\
% V219 & 0.61361 & 0.00001 & RRab & 15.996 & 0.884 & 16.043 & 0.940 & 15.674 & 0.763 & 15.454 & 0.445 & 15.104 & 0.508 & -- & Bl & BAACA \\
% V220 & 0.60011 & 0.00001 & RRab & 15.954 & 0.658 & 15.988 & 0.899 & 15.606 & 0.793 & 15.354 & 0.698 & 14.966 & 0.424 & -- & Bl & AABCA \\
% V221 & 0.37877 & 0.00003 & RRc & 15.353 & 0.615 & 15.437 & 0.663 & 15.190 & 0.574 & 15.031 & 0.419 & 14.831 & 0.397 & -- & -- & BAACA \\
% V222 & 0.59674 & 0.00004 & RRab & 15.786 & 0.871 & 15.939 & 1.036 & 15.558 & 0.732 & 15.175 & 0.601 & 15.041 & 0.418 & OoI & -- & AAACA \\
% V223 & 0.32923 & 0.00003 & RRc & 15.632 & 0.772 & 15.684 & 0.833 & 15.433 & 0.721 & 15.355 & 0.527 & 15.163 & 0.499 & -- & -- & BAACA \\
% V226 & 0.48843 & 0.00003 & RRab & 15.771 & 1.237 & 15.699 & 1.230 & 15.445 & 0.908 & 15.322 & 0.904 & 15.072 & 0.707 & -- & -- & ACBCA \\
% V229 & 0.49762 & 0.01848 & RRab & 15.883 & 1.663 & 15.881 & 1.573 & 15.593 & 1.159 & 15.565 & 0.750 & 15.166 & 0.790 & -- & -- & BAACB \\
% V234 & 0.50802 & 0.00002 & RRab & 16.110 & 1.382 & 15.937 & 1.127 & 15.614 & 0.923 & 15.352 & 0.648 & 15.295 & 0.618 & -- & -- & ABBCA \\
% V235 & 0.75984 & 0.00004 & RRab & 15.790 & 0.601 & 15.844 & 0.548 & 15.447 & 0.477 & 15.105 & 0.320 & 14.856 & 0.278 & OoII & -- & AAACA \\
% V239 & 0.50398 & 0.00002 & RRab & 15.930 & 1.022 & 15.971 & 1.292 & 15.654 & 0.915 & 15.523 & 0.940 & 15.203 & 0.763 & -- & Bl & CAACB \\
% V240 & 0.27601 & 0.00001 & RRc & 15.548 & 0.565 & 15.565 & 0.610 & 15.252 & 0.528 & 14.996 & 0.578 & 14.768 & 0.365 & -- & -- & AAACA \\
% V241 & 0.59617 & 0.00003 & RRab & 15.805 & 1.291 & 15.818 & 1.457 & 15.503 & 1.154 & 15.330 & 0.879 & 15.033 & 0.844 & -- & -- & BAACA \\
% V242 & 0.59650 & 0.00010 & RRab & 15.602 & 0.846 & 15.818 & 0.731 & 15.451 & 0.574 & 15.310 & 0.377 & 14.955 & 0.389 & -- & -- & AAACA \\
% V243 & 0.63462 & 0.00002 & RRab & 15.778 & 0.877 & 15.879 & 0.673 & 15.482 & 0.554 & 15.225 & 0.536 & 14.861 & 0.373 & -- & Bl & AAACA \\
% V244 & 0.53784 & 0.00004 & RRab & 15.766 & 1.215 & 15.839 & 1.301 & 15.553 & 1.090 & 15.347 & 1.076 & 15.200 & 0.832 & -- & -- & ACCCB \\
% V245 & 0.28403 & 0.00003 & RRc & 15.707 & 0.765 & 15.764 & 0.825 & 15.492 & 0.715 & 15.476 & 0.522 & 15.188 & 0.495 & -- & -- & AAACA \\
% V246 & 0.33914 & 0.00004 & RRc & 15.705 & 0.770 & 15.762 & 0.830 & 15.496 & 0.719 & 15.309 & 0.525 & 15.095 & 0.498 & -- & -- & BAACA \\
% V247 & 0.60536 & 0.00004 & RRab & 15.921 & 0.893 & 16.077 & 0.889 & 15.671 & 0.769 & 15.429 & 0.651 & 15.052 & 0.497 & -- & -- & BABCB \\
% V248 & 0.50979 & 0.00001 & RRab & 15.730 & 0.996 & 15.859 & 1.001 & 15.589 & 0.813 & 15.426 & 0.554 & 15.030 & 0.541 & -- & -- & BBACB \\
% V249 & 0.53300 & 0.00001 & RRab & 15.400 & 1.206 & 15.406 & 0.936 & 15.086 & 0.722 & 14.777 & 0.500 & 14.612 & 0.475 & -- & -- & BBBCB \\
% V250n & 0.57438 & 0.00438 & RRab & 16.023 & 1.014 & 16.064 & 1.160 & 15.710 & 0.950 & 15.421 & 1.047 & 15.120 & 0.574 & -- & -- & AAACA \\
% V250s & 0.59242 & 0.00242 & RRab & 15.638 & 0.838 & 15.847 & 0.964 & 15.462 & 0.791 & 15.334 & 0.527 & 15.012 & 0.530 & -- & -- & BAACA \\
% V251 & 0.35392 & 0.00028 & RRd & 15.260 & 0.632 & 15.300 & 0.682 & 15.112 & 0.836 & 14.976 & 0.431 & 14.861 & 0.409 & -- & -- & BBBCA \\
% V252 & 0.30350 & 0.03260 & RRd & 15.804 & 0.708 & 15.718 & 0.764 & 15.467 & 0.661 & 15.475 & 0.483 & 15.196 & 0.458 & -- & -- & BBBCB \\
% V253 & 0.33262 & 0.00002 & RRc & 15.393 & 0.677 & 15.518 & 0.730 & 15.281 & 0.633 & 15.120 & 0.473 & 14.913 & 0.438 & -- & -- & AAACA \\
% V254 & 0.60564 & 0.00006 & RRab & 15.680 & 0.930 & 15.796 & 0.992 & 15.396 & 0.748 & 15.425 & 0.555 & 15.010 & 0.542 & -- & -- & BCBCB \\
% V255 & 0.57271 & 0.00001 & RRab & 15.794 & 0.752 & 15.860 & 0.833 & 15.440 & 0.595 & 15.148 & 0.418 & 14.864 & 0.392 & -- & Bl & AAACA \\
% V256 & 0.31805 & 0.00005 & RRc & 15.894 & 0.937 & 15.857 & 1.011 & 15.644 & 0.876 & 15.456 & 0.639 & 15.295 & 0.606 & -- & -- & ABBCA \\
% V257 & 0.60206 & 0.00006 & RRab & 15.698 & 0.818 & 15.768 & 0.886 & 15.425 & 0.705 & 15.300 & 0.751 & 14.916 & 0.426 & -- & -- & AAACA \\
% V258 & 0.71340 & 0.00000 & RRab & 15.896 & 0.632 & 15.971 & 0.649 & 15.584 & 0.500 & 15.334 & 0.439 & 15.001 & 0.321 & -- & -- & AAACA \\
% V259 & 0.33352 & 0.00002 & RRc & 15.481 & 0.399 & 15.501 & 0.431 & 15.080 & 0.373 & 14.815 & 0.272 & 14.467 & 0.258 & -- & -- & AAACA \\
% V261 & 0.44467 & 0.00023 & RRc & 15.146 & 0.988 & 15.188 & 1.065 & 14.875 & 0.923 & 14.631 & 0.674 & 14.538 & 0.639 & -- & -- & BBBCB \\
% V262 & 0.65505 & 0.00005 & RRab & 15.664 & 0.527 & 15.880 & 0.569 & 15.479 & 0.467 & 15.439 & 0.294 & 15.015 & 0.261 & -- & -- & BBBCA \\
% V264 & 0.35647 & 0.00003 & RRc & 15.700 & 0.879 & 15.647 & 0.948 & 15.287 & 0.821 & 15.228 & 0.600 & 14.946 & 0.568 & -- & -- & ABBCA \\
% V266 & 0.34244 & 0.00006 & RRc & 15.630 & 0.562 & 15.710 & 0.606 & 15.411 & 0.525 & 15.234 & 0.575 & 14.967 & 0.358 & -- & -- & AAACA \\
V269 & 0.35570 & 0.00430 & RRc & 15.212 & 0.625 & 15.329 & 0.674 & 15.062 & 0.553 & 14.988 & 0.640 & 14.807 & 0.404 & -- & -- & BABCB \\
V270n & 0.62586 & 0.00414 & RRab & 15.740 & 0.653 & 15.814 & 0.799 & 15.457 & 0.659 & 15.254 & 0.563 & 14.930 & 0.386 & -- & -- & AAACA \\
V270s & 0.69019 & 0.00019 & RRab & 15.041 & 1.059 & 15.088 & 1.195 & 14.873 & 0.861 & 14.558 & 0.624 & 14.514 & 0.620 & -- & -- & AAACA \\
V271 & 0.63280 & 0.00000 & RRab & 16.084 & 0.817 & 16.088 & 0.807 & 15.674 & 0.594 & 15.403 & 0.340 & 15.069 & 0.367 & -- & -- & AAACA \\
V290 & 0.24041 & 0.00001 & RRd & 15.881 & 0.115 & 15.851 & 0.124 & 15.674 & 0.107 & 15.547 & 0.078 & 15.374 & 0.074 & -- & -- & AAACA \\
V292 & 0.29654 & 0.00006 & RRc & 15.785 & 0.472 & 15.778 & 0.509 & 15.603 & 0.441 & 15.501 & 0.322 & 15.331 & 0.305 & -- & -- & AAACA \\
\hline
\end{tabular}

==> tables/table_2_long_copy.tex <==
% \begin{longtable}{ccccccccccccccc}
% \hline
% Star & Period & Type & <U> & $A_U$ & <B> &$ A_B$ & <V> & $A_V $& <R> & $A_R$ & <I> & $A_I$ & Oo type & Blazhko \\
%  & days &  & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ &  &  \\
%  \hline
% \endfirsthead
% % Table header for subsequent pages
% \multicolumn{3}{c}{\tablename~\thetable{} -- continued from previous page} \\
% \hline
% Star & Period & Type & <U> & $A_U$ & <B> &$ A_B$ & <V> & $A_V $& <R> & $A_R$ & <I> & $A_I$ & Oo type & Blazhko \\
%  & days &  & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ & $\mathrm{mag}$ &  &  \\
% \hline
% \endhead
% 
V1 & 0.52059 & RRab & 15.470 & 0.635 & 16.221 & 0.694 & 15.824 & 0.568 & 15.525 & 0.441 & 15.266 & 0.356 & OoI &  \\
V3 & 0.55820 & RRab & 15.738 & 1.478 & 15.969 & 1.346 & 15.606 & 0.974 & 15.289 & 0.733 & 15.117 & 0.743 & OoII & Bl \\
V4n & 0.58504 & RRab & 15.074 & 0.808 & 15.114 & 0.932 & 14.754 & 0.763 & 14.430 & 0.595 & 14.205 & 0.487 &  &  \\
V5 & 0.50583 & RRab & 15.990 & 1.008 & 16.028 & 1.366 & 15.691 & 1.053 & 15.507 & 0.580 & 15.216 & 0.781 & OoI & Bl \\
V6 & 0.51434 & RRab & 16.012 & 1.419 & 16.045 & 1.268 & 15.693 & 1.130 & 15.498 & 0.715 & 15.243 & 0.813 & OoI &  \\
V7 & 0.49742 & RRab & 15.679 & 0.794 & 15.678 & 0.881 & 15.394 & 0.606 & 15.212 & 0.495 & 15.163 & 0.499 & OoI & Bl \\
V8 & 0.63672 & RRab & 15.684 & 0.648 & 15.735 & 0.851 & 15.273 & 0.585 & 14.913 & 0.401 & 14.566 & 0.236 &  & Bl \\
V9 & 0.55666 & RRab & 16.272 & 0.969 & 15.928 & 1.291 & 15.643 & 1.019 & 15.601 & 0.502 & 15.181 & 0.783 & OoI &  \\
V10 & 0.56955 & RRab & 15.975 & 1.103 & 16.051 & 1.106 & 15.719 & 0.748 & 15.402 & 0.593 & 15.153 & 0.512 & OoI & Bl \\
V11 & 0.50789 & RRab & 15.395 & 1.119 & 16.032 & 1.577 & 15.712 & 1.191 & 15.450 & 1.011 & 15.224 & 0.831 & OoI &  \\
V12 & 0.32557 & RRc & 15.896 & 0.501 & 15.871 & 0.540 & 15.633 & 0.468 & 15.597 & 0.342 & 15.306 & 0.324 &  &  \\
V13 & 0.32350 & RRd & 16.109 & 0.787 & 16.001 & 0.849 & 15.644 & 0.735 & 15.570 & 0.537 & 15.232 & 0.509 &  & Bl \\
V14 & 0.63590 & RRab & 15.910 & 1.315 & 15.901 & 1.278 & 15.550 & 1.004 & 15.169 & 0.882 & 15.054 & 0.556 & OoII & Bl \\
V15 & 0.53009 & RRab & 16.097 & 0.919 & 16.063 & 1.129 & 15.766 & 0.851 & 15.447 & 0.922 & 15.182 & 0.716 & OoI &  \\
V16 & 0.51149 & RRab & 16.054 & 1.465 & 16.103 & 1.460 & 15.766 & 1.134 & 15.546 & 1.008 & 15.270 & 0.827 & OoI &  \\
V17 & 0.57616 & RRab & 16.014 & 0.833 & 16.028 & 0.878 & 15.699 & 0.717 & 15.437 & 0.460 & 15.166 & 0.425 & OoI & Bl \\
V18 & 0.51645 & RRab & 16.089 & 1.429 & 16.168 & 1.059 & 15.816 & 0.911 & 15.499 & 0.888 & 15.310 & 0.567 & OoI &  \\
V19 & 0.63197 & RRab & 16.081 & 0.653 & 16.107 & 0.579 & 15.722 & 0.435 & 15.442 & 0.387 & 15.156 & 0.288 & OoI &  \\
V20 & 0.49752 & RRab & 15.805 & 1.131 & 15.979 & 1.228 & 15.558 & 1.308 & 15.460 & 0.651 & 15.130 & 0.602 & OoI & Bl \\
V21 & 0.51367 & RRab & 16.026 & 0.934 & 16.158 & 1.180 & 15.776 & 0.875 & 15.620 & 0.493 & 15.203 & 0.452 & OoI &  \\
V22 & 0.48141 & RRab & 15.839 & 1.160 & 16.069 & 1.331 & 15.695 & 1.323 & 15.562 & 0.626 & 15.264 & 0.617 & OoI & Bl \\
V23 & 0.59538 & RRab & 15.865 & 0.961 & 16.055 & 0.944 & 15.681 & 0.763 & 15.291 & 0.550 & 15.143 & 0.460 & OoI & Bl \\
V24 & 0.66340 & RRab & 15.908 & 0.902 & 15.928 & 1.090 & 15.560 & 0.825 & 15.213 & 0.434 & 15.027 & 0.431 & OoII & Bl \\
V25 & 0.48006 & RRab & 16.010 & 1.426 & 16.157 & 1.312 & 15.713 & 1.116 & 15.532 & 1.050 & 15.264 & 0.683 & OoI &  \\
V26 & 0.59774 & RRab & 15.922 & 1.184 & 15.961 & 1.177 & 15.618 & 0.906 & 15.374 & 0.788 & 15.089 & 0.668 & OoII &  \\
V27 & 0.57906 & RRab & 15.964 & 1.066 & 16.018 & 1.102 & 15.661 & 0.840 & 15.401 & 0.781 & 15.145 & 0.568 & OoI &  \\
V28 & 0.47064 & RRab & 15.934 & 1.223 & 15.960 & 1.378 & 15.690 & 1.053 & 15.511 & 0.793 & 15.247 & 0.640 & OoI & Bl \\
V29 & 0.47178 & RRab & 15.773 & 1.060 & 15.895 & 1.171 & 15.576 & 0.970 & 15.405 & 0.649 & 15.193 & 0.653 &  &  \\
V30 & 0.51209 & RRab & 16.199 & 1.018 & 15.978 & 1.254 & 15.633 & 1.018 & 15.421 & 0.846 & 15.171 & 0.696 &  &  \\
V31 & 0.58073 & RRab & 15.830 & 1.410 & 15.890 & 1.377 & 15.570 & 1.140 & 15.163 & 0.805 & 15.085 & 0.710 & OoII &  \\
V32 & 0.49535 & RRab & 16.093 & 0.896 & 15.930 & 1.382 & 15.613 & 1.100 & 15.513 & 0.627 & 15.106 & 0.698 & OoI &  \\
V33 & 0.52525 & RRab & 15.832 & 1.080 & 15.994 & 1.138 & 15.671 & 0.932 & 15.552 & 0.652 & 15.174 & 0.610 & OoI & Bl \\
V34 & 0.55910 & RRab & 16.012 & 0.746 & 16.072 & 0.903 & 15.718 & 0.743 & 15.372 & 0.694 & 15.203 & 0.440 & OoI & Bl \\
V35 & 0.52976 & RRab & 15.919 & 1.208 & 16.040 & 1.354 & 15.723 & 1.110 & 15.465 & 0.730 & 15.242 & 0.633 & OoI & Bl \\
V36 & 0.54559 & RRab & 15.931 & 1.402 & 16.075 & 1.285 & 15.729 & 1.011 & 15.341 & 0.556 & 15.206 & 0.752 & OoI &  \\
V37 & 0.32664 & RRc & 15.927 & 0.604 & 15.898 & 0.651 & 15.669 & 0.564 & 15.479 & 0.423 & 15.290 & 0.390 &  &  \\
V38 & 0.55801 & RRab & 15.995 & 1.253 & 16.066 & 0.972 & 15.716 & 0.706 & 15.353 & 0.496 & 15.222 & 0.471 & OoI & Bl \\
V39 & 0.58707 & RRab & 16.078 & 0.696 & 16.023 & 0.906 & 15.669 & 0.710 & 15.459 & 0.422 & 15.169 & 0.503 & OoI & Bl \\
V40 & 0.55154 & RRab & 16.042 & 1.184 & 16.104 & 1.207 & 15.738 & 0.945 & 15.335 & 0.882 & 15.240 & 0.600 & OoI &  \\
V41 & 0.48509 & RRab & 16.014 & 1.435 & 16.010 & 1.511 & 15.626 & 1.067 & 15.476 & 0.862 & 15.275 & 0.586 & OoI & Bl \\
V42 & 0.59008 & RRab & 15.787 & 1.240 & 15.750 & 1.338 & 15.457 & 1.009 & 15.432 & 0.595 & 15.059 & 0.765 & OoII &  \\
V43 & 0.54052 & RRab & 16.022 & 1.397 & 16.032 & 1.337 & 15.711 & 1.050 & 15.458 & 0.823 & 15.189 & 0.674 &  & Bl \\
V44 & 0.36810 & RRd & 15.775 & 0.821 & 16.051 & 0.885 & 15.606 & 0.767 & 15.113 & 0.560 & 15.271 & 0.531 &  & Bl \\
V45 & 0.53691 & RRab & 16.248 & 0.969 & 16.229 & 1.036 & 15.784 & 0.849 & 15.570 & 0.725 & 15.291 & 0.557 & OoI & Bl \\
V46 & 0.61339 & RRab & 16.036 & 0.758 & 16.108 & 0.688 & 15.712 & 0.500 & 15.425 & 0.374 & 15.149 & 0.361 & OoI &  \\
V47 & 0.57257 & RRab & 15.927 & 0.890 & 15.923 & 0.952 & 15.594 & 0.780 & 15.506 & 0.448 & 15.192 & 0.531 & OoI & Bl \\
V48 & 0.62784 & RRab & 15.893 & 0.597 & 15.935 & 0.685 & 15.544 & 0.506 & 15.245 & 0.392 & 14.959 & 0.378 & OoI? & Bl \\
V49 & 0.54821 & RRab & 15.938 & 1.113 & 15.920 & 1.105 & 15.544 & 0.944 & 15.409 & 0.652 & 15.170 & 0.628 & OoI & Bl \\
V50 & 0.51310 & RRab & 16.096 & 1.300 & 16.063 & 1.268 & 15.672 & 1.117 & 15.513 & 0.767 & 15.257 & 0.590 & OoI & Bl \\
V51 & 0.58397 & RRab & 16.001 & 0.940 & 16.042 & 1.035 & 15.691 & 0.811 & 15.391 & 0.592 & 15.150 & 0.585 & OoI &  \\
V52 & 0.51624 & RRab & 16.188 & 1.204 & 15.965 & 1.249 & 15.674 & 0.899 & 15.459 & 0.631 & 15.247 & 0.802 & OoI & Bl \\
V53 & 0.50488 & RRab & 16.298 & 0.435 & 16.358 & 0.469 & 15.994 & 0.396 & 15.656 & 0.249 & 15.286 & 0.248 & OoI &  \\
V54 & 0.50620 & RRab & 16.056 & 0.836 & 16.170 & 0.942 & 15.779 & 0.727 & 15.523 & 0.712 & 15.239 & 0.420 & OoI & Bl \\
V55 & 0.52983 & RRab & 16.150 & 1.209 & 16.013 & 1.094 & 15.683 & 0.895 & 15.447 & 0.774 & 15.228 & 0.717 & OoI &  \\
V56 & 0.32960 & RRc & 15.874 & 0.553 & 15.926 & 0.579 & 15.648 & 0.468 & 15.469 & 0.404 & 15.278 & 0.304 &  &  \\
V57 & 0.51218 & RRab & 16.143 & 1.099 & 16.116 & 1.214 & 15.753 & 0.968 & 15.564 & 0.779 & 15.184 & 0.583 & OoI &  \\
V58 & 0.51705 & RRab & 15.999 & 1.600 & 15.858 & 1.455 & 15.619 & 1.151 & 15.409 & 0.685 & 15.190 & 0.827 & OoI &  \\
V59 & 0.58883 & RRab & 16.062 & 0.970 & 16.076 & 0.927 & 15.693 & 0.744 & 15.459 & 0.543 & 15.182 & 0.466 & OoI & Bl \\
V60 & 0.70773 & RRab & 15.956 & 0.844 & 15.949 & 0.845 & 15.566 & 0.646 & 15.344 & 0.603 & 15.012 & 0.415 & OoII &  \\
V61 & 0.52089 & RRab & 16.051 & 1.097 & 16.119 & 1.004 & 15.738 & 0.732 & 15.589 & 0.434 & 15.196 & 0.571 &  &  \\
V62 & 0.65240 & RRab & 16.002 & 0.675 & 16.045 & 0.668 & 15.645 & 0.490 & 15.384 & 0.515 & 15.079 & 0.323 & OoI & Bl \\
V63 & 0.57040 & RRab & 16.025 & 1.215 & 16.076 & 1.232 & 15.722 & 0.889 & 15.523 & 0.580 & 15.189 & 0.586 & OoI & Bl \\
V64 & 0.60546 & RRab & 16.066 & 0.841 & 16.101 & 0.945 & 15.714 & 0.711 & 15.461 & 0.607 & 15.158 & 0.444 & OoI &  \\
V65 & 0.66716 & RRab & 16.057 & 0.999 & 15.959 & 1.156 & 15.582 & 0.946 & 15.377 & 0.527 & 15.010 & 0.592 & OoII &  \\
V66 & 0.62019 & RRab & 16.010 & 0.705 & 16.060 & 0.784 & 15.657 & 0.615 & 15.412 & 0.461 & 15.125 & 0.366 & OoI & Bl \\
V67 & 0.56833 & RRab & 16.041 & 0.704 & 16.113 & 0.854 & 15.720 & 0.746 & 15.479 & 0.617 & 15.193 & 0.476 & OoI & Bl \\
V68 & 0.36053 & RRd & 15.932 & 0.675 & 15.823 & 0.728 & 15.528 & 0.630 & 15.411 & 0.460 & 15.222 & 0.436 &  &  \\
V69 & 0.56662 & RRab & 16.113 & 1.087 & 16.089 & 1.157 & 15.730 & 0.899 & 15.448 & 0.698 & 15.193 & 0.545 & OoI &  \\
V70 & 0.48606 & RRc & 15.576 & 0.360 & 15.675 & 0.425 & 15.368 & 0.340 & 15.168 & 0.253 & 14.921 & 0.232 &  & Bl \\
V71 & 0.54905 & RRab & 15.958 & 1.132 & 16.083 & 1.166 & 15.725 & 0.905 & 15.511 & 0.705 & 15.181 & 0.531 & OoI & Bl \\
V72 & 0.45608 & RRab & 15.839 & 1.487 & 15.945 & 1.461 & 15.716 & 1.190 & 15.293 & 0.882 & 15.332 & 0.726 & OoI &  \\
V73 & 0.67348 & RRab & 16.001 & 0.430 & 16.073 & 0.350 & 15.671 & 0.272 & 15.348 & 0.227 & 15.074 & 0.155 & OoI & Bl \\
V74 & 0.49216 & RRab & 16.070 & 1.528 & 16.060 & 1.633 & 15.671 & 1.350 & 15.570 & 0.850 & 15.285 & 0.713 & OoI &  \\
V75 & 0.31408 & RRc & 15.913 & 0.554 & 15.936 & 0.578 & 15.686 & 0.489 & 15.518 & 0.357 & 15.303 & 0.338 &  &  \\
V76 & 0.50176 & RRab & 15.938 & 1.591 & 16.049 & 1.518 & 15.720 & 1.203 & 15.331 & 0.582 & 15.266 & 0.724 & OoI &  \\
V77 & 0.45935 & RRab & 16.397 & 0.855 & 15.999 & 1.133 & 15.805 & 1.015 & 15.783 & 0.586 & 15.446 & 0.559 & OoI & Bl \\
V78 & 0.61191 & RRab & 15.855 & 0.970 & 16.017 & 0.812 & 15.667 & 0.607 & 15.413 & 0.395 & 15.086 & 0.381 & OoII? & Bl \\
V79 & 0.48326 & RRab & 16.161 & 0.893 & 16.187 & 0.973 & 15.910 & 0.790 & 15.513 & 0.469 & 15.337 & 0.466 & OoI & Bl \\
V80 & 0.52906 & RRab & 16.022 & 0.809 & 16.254 & 0.899 & 15.739 & 0.852 & 15.401 & 0.572 & 15.293 & 0.521 & OoI & Bl \\
V81 & 0.52912 & RRab & 15.812 & 1.393 & 16.132 & 1.199 & 15.706 & 1.083 & 15.450 & 0.675 & 15.216 & 0.730 & OoI &  \\
V82 & 0.52454 & RRab & 16.035 & 1.438 & 16.078 & 1.355 & 15.744 & 1.061 & 15.475 & 0.948 & 15.228 & 0.719 & OoI &  \\
V83 & 0.50127 & RRab & 16.092 & 0.979 & 16.141 & 1.320 & 15.766 & 0.952 & 15.692 & 0.512 & 15.287 & 0.859 & OoI &  \\
V84 & 0.59573 & RRab & 15.985 & 1.018 & 16.064 & 0.933 & 15.704 & 0.698 & 15.394 & 0.633 & 15.145 & 0.486 & OoI &  \\
V85 & 0.35581 & RRc & 15.835 & 0.538 & 15.740 & 0.546 & 15.512 & 0.430 & 15.360 & 0.314 & 15.154 & 0.297 &  &  \\
V86 & 0.29266 & RRc & 15.948 & 0.484 & 15.899 & 0.645 & 15.695 & 0.498 & 15.490 & 0.330 & 15.327 & 0.313 &  &  \\
V87 & 0.35748 & RRd & 15.846 & 0.510 & 15.871 & 0.550 & 15.593 & 0.476 & 15.299 & 0.348 & 15.146 & 0.329 &  &  \\
V88 & 0.29875 & RRc & 15.940 & 0.703 & 15.922 & 0.758 & 15.701 & 0.657 & 15.415 & 0.480 & 15.370 & 0.454 &  &  \\
V89 & 0.54848 & RRab & 16.042 & 1.107 & 16.004 & 1.309 & 15.663 & 0.999 & 15.388 & 0.743 & 15.139 & 0.624 & OoI &  \\
V90 & 0.51703 & RRab & 16.000 & 1.370 & 16.078 & 1.356 & 15.782 & 1.055 & 15.543 & 0.850 & 15.234 & 0.751 & OoI &  \\
V91 & 0.53011 & RRab & 15.859 & 1.018 & 16.066 & 1.168 & 15.702 & 0.804 & 15.409 & 0.770 & 15.202 & 0.479 & OoI & Bl \\
V92 & 0.50355 & RRab & 15.964 & 0.874 & 16.113 & 0.814 & 15.783 & 0.677 & 15.481 & 0.448 & 15.415 & 0.447 & OoI & Bl \\
V93 & 0.60230 & RRab & 15.935 & 0.830 & 16.108 & 0.896 & 15.718 & 0.667 & 15.529 & 0.644 & 15.183 & 0.502 & OoI &  \\
V94 & 0.52370 & RRab & 16.335 & 0.899 & 15.948 & 1.042 & 15.720 & 0.848 & 15.493 & 0.546 & 15.298 & 0.541 & OoI &  \\
V96 & 0.49941 & RRab & 15.624 & 0.769 & 16.234 & 0.985 & 15.858 & 0.813 & 15.529 & 0.705 & 15.377 & 0.699 & OoI &  \\
V97 & 0.33493 & RRc & 16.059 & 0.392 & 15.976 & 0.508 & 15.710 & 0.409 & 15.518 & 0.343 & 15.311 & 0.254 &  &  \\
V99 & 0.35543 & RRd & 15.760 & 0.526 & 15.913 & 0.567 & 15.665 & 0.491 & 15.375 & 0.391 & 15.158 & 0.340 &  & Bl \\
V100 & 0.61881 & RRab & 15.988 & 0.657 & 16.177 & 0.583 & 15.744 & 0.502 & 15.452 & 0.489 & 15.101 & 0.273 & OoI &  \\
V101 & 0.64389 & RRab & 16.013 & 0.645 & 16.065 & 0.652 & 15.669 & 0.537 & 15.370 & 0.364 & 15.110 & 0.359 & OoI & Bl \\
V104 & 0.56993 & RRab & 15.832 & 1.424 & 15.917 & 1.421 & 15.610 & 1.127 & 15.362 & 0.852 & 15.110 & 0.706 & OoII & Bl \\
V105 & 0.28775 & RRc & 15.866 & 0.408 & 15.819 & 0.440 & 15.619 & 0.381 & 15.440 & 0.287 & 15.334 & 0.264 &  &  \\
V106 & 0.53725 & RRab & 16.016 & 0.745 & 16.040 & 0.876 & 15.695 & 0.661 & 15.492 & 0.379 & 15.234 & 0.444 & OoI & Bl \\
V107 & 0.30903 & RRc & 16.089 & 0.490 & 15.874 & 0.528 & 15.664 & 0.458 & 15.312 & 0.334 & 15.342 & 0.317 &  &  \\
V108 & 0.51961 & RRab & 16.080 & 1.414 & 16.084 & 1.376 & 15.764 & 1.079 & 15.546 & 0.646 & 15.273 & 0.745 & OoI &  \\
V109 & 0.53392 & RRab & 16.109 & 1.270 & 16.064 & 1.422 & 15.706 & 1.057 & 15.295 & 0.752 & 15.202 & 0.754 & OoI &  \\
V110 & 0.53546 & RRab & 16.034 & 0.970 & 16.009 & 1.127 & 15.671 & 0.924 & 15.375 & 0.688 & 15.168 & 0.617 & OoI & Bl \\
V111 & 0.51019 & RRab & 15.866 & 1.108 & 16.070 & 1.065 & 15.738 & 0.923 & 15.345 & 0.566 & 15.246 & 0.557 & OoI & Bl \\
V113 & 0.51300 & RRab & 16.200 & 1.095 & 15.981 & 1.497 & 15.674 & 1.196 & 15.502 & 0.574 & 15.153 & 0.654 & OoI &  \\
V114 & 0.59772 & RRab & 15.981 & 1.012 & 16.092 & 0.972 & 15.693 & 0.780 & 15.467 & 0.539 & 15.154 & 0.456 & OoI & Bl \\
V115 & 0.51335 & RRab & 15.821 & 1.352 & 16.039 & 1.527 & 15.710 & 1.188 & 15.387 & 0.736 & 15.236 & 0.742 & OoI &  \\
V116 & 0.51481 & RRab & 16.074 & 1.338 & 15.999 & 1.326 & 15.696 & 1.040 & 15.499 & 0.807 & 15.274 & 0.741 & OoI &  \\
V117 & 0.60054 & RRab & 16.076 & 1.100 & 15.994 & 1.209 & 15.649 & 0.836 & 15.427 & 0.675 & 15.125 & 0.583 & OoI & Bl \\
V118 & 0.49940 & RRab & 16.476 & 1.150 & 15.968 & 1.538 & 15.737 & 1.212 & 15.728 & 0.668 & 15.278 & 0.809 &  &  \\
V119 & 0.51835 & RRab & 16.177 & 1.106 & 15.910 & 1.269 & 15.673 & 0.969 & 15.331 & 0.566 & 15.242 & 0.666 & OoI & Bl \\
V120 & 0.64014 & RRab & 16.048 & 0.547 & 16.091 & 0.583 & 15.699 & 0.404 & 15.399 & 0.241 & 15.128 & 0.302 & OoI &  \\
V121 & 0.53521 & RRab & 16.022 & 1.320 & 16.039 & 1.242 & 15.708 & 0.928 & 15.466 & 0.640 & 15.167 & 0.656 & OoI & Bl \\
V122 & 0.51093 & RRab & 16.196 & 1.048 & 16.114 & 1.301 & 15.711 & 1.166 & 15.657 & 0.922 & 15.255 & 0.661 &  &  \\
V123 & 0.54548 & RRab & 16.040 & 1.267 & 15.981 & 1.306 & 15.659 & 1.046 & 15.434 & 0.610 & 15.194 & 0.719 & OoI &  \\
V124 & 0.75244 & RRab & 15.920 & 0.517 & 15.967 & 0.459 & 15.566 & 0.356 & 15.268 & 0.290 & 14.982 & 0.229 & OoII &  \\
V125 & 0.34982 & RRd & 15.900 & 0.486 & 15.963 & 0.496 & 15.707 & 0.368 & 15.487 & 0.288 & 15.225 & 0.255 &  &  \\
V126 & 0.34840 & RRc & 15.951 & 0.428 & 15.972 & 0.462 & 15.686 & 0.400 & 15.440 & 0.193 & 15.244 & 0.277 &  & Bl \\
V128 & 0.29204 & RRc & 15.880 & 0.540 & 15.878 & 0.651 & 15.654 & 0.535 & 15.551 & 0.363 & 15.311 & 0.344 &  &  \\
V130 & 0.55904 & RRab & 15.851 & 0.829 & 15.975 & 0.861 & 15.603 & 0.710 & 15.384 & 0.474 & 15.107 & 0.421 & OoI & Bl \\
V131 & 0.29769 & RRc & 15.840 & 0.558 & 15.865 & 0.631 & 15.640 & 0.506 & 15.520 & 0.488 & 15.277 & 0.351 &  &  \\
V132 & 0.33986 & RRc & 15.814 & 0.467 & 15.893 & 0.453 & 15.621 & 0.380 & 15.509 & 0.278 & 15.209 & 0.263 &  &  \\
V133 & 0.55073 & RRab & 16.187 & 0.996 & 15.906 & 1.064 & 15.725 & 0.977 & 15.523 & 0.600 & 15.198 & 0.587 & OoI & Bl \\
V134 & 0.61806 & RRab & 15.943 & 0.798 & 16.049 & 0.784 & 15.655 & 0.574 & 15.454 & 0.482 & 15.102 & 0.392 &  &  \\
V135 & 0.56839 & RRab & 15.709 & 0.899 & 16.022 & 1.168 & 15.661 & 0.885 & 15.393 & 0.585 & 15.129 & 0.608 & OoI & Bl \\
V136 & 0.61718 & RRab & 15.793 & 0.800 & 15.909 & 0.797 & 15.520 & 0.632 & 15.203 & 0.628 & 14.956 & 0.405 &  &  \\
V137 & 0.57515 & RRab & 15.837 & 1.114 & 15.986 & 1.088 & 15.620 & 0.879 & 15.315 & 0.486 & 15.099 & 0.481 & OoI &  \\
V139 & 0.55999 & RRab & 15.784 & 1.408 & 15.849 & 1.347 & 15.484 & 1.098 & 15.217 & 1.036 & 15.044 & 0.822 &  &  \\
V140 & 0.33314 & RRc & 15.698 & 0.475 & 15.731 & 0.529 & 15.499 & 0.418 & 15.264 & 0.352 & 15.132 & 0.272 &  & Bl \\
V142 & 0.56863 & RRab & 15.974 & 1.198 & 16.094 & 1.219 & 15.710 & 0.968 & 15.477 & 0.826 & 15.203 & 0.644 & OoI &  \\
V143 & 0.59654 & RRab & 15.473 & 0.980 & 15.895 & 0.848 & 15.435 & 0.703 & 15.202 & 0.481 & 14.809 & 0.503 & OoII & Bl \\
V144 & 0.59679 & RRab & 15.946 & 0.583 & 15.994 & 0.618 & 15.601 & 0.506 & 15.281 & 0.346 & 15.058 & 0.344 &  &  \\
V145 & 0.51449 & RRab & 15.627 & 0.998 & 15.755 & 1.116 & 15.408 & 0.841 & 15.045 & 0.533 & 14.875 & 0.576 &  &  \\
V146 & 0.50220 & RRab & 15.754 & 1.079 & 15.972 & 1.178 & 15.659 & 0.915 & 15.579 & 0.894 & 15.192 & 0.669 & OoI &  \\
V147 & 0.34648 & RRc & 15.836 & 0.475 & 15.954 & 0.514 & 15.657 & 0.444 & 15.448 & 0.424 & 15.260 & 0.307 &  &  \\
V148 & 0.46727 & RRab & 16.158 & 1.314 & 16.200 & 1.654 & 15.808 & 1.497 & 15.453 & 1.460 & 15.354 & 1.030 &  &  \\
V149 & 0.54818 & RRab & 16.099 & 0.952 & 15.931 & 1.298 & 15.622 & 0.971 & 15.381 & 0.595 & 15.140 & 0.520 &  & Bl \\
V150 & 0.52392 & RRab & 15.744 & 1.246 & 16.028 & 1.252 & 15.674 & 1.000 & 15.529 & 0.743 & 15.211 & 0.638 & OoI & Bl \\
V151 & 0.51682 & RRab & 15.630 & 0.913 & 16.038 & 1.009 & 15.660 & 0.825 & 15.507 & 0.555 & 15.148 & 0.571 &  & Bl \\
V152 & 0.32613 & RRc & 15.712 & 0.480 & 15.697 & 0.517 & 15.493 & 0.448 & 15.328 & 0.327 & 15.179 & 0.310 &  &  \\
V155 & 0.33232 & RRc & 15.758 & 0.702 & 15.793 & 0.757 & 15.544 & 0.656 & 15.298 & 0.479 & 15.177 & 0.454 &  &  \\
V156 & 0.53199 & RRab & 15.776 & 1.204 & 15.836 & 1.280 & 15.501 & 0.988 & 15.225 & 0.805 & 15.032 & 0.626 &  &  \\
V157 & 0.54284 & RRab & 15.465 & 0.659 & 16.111 & 0.710 & 15.634 & 0.610 & 15.144 & 0.381 & 14.920 & 0.386 &  & Bl \\
V159 & 0.53380 & RRab & 15.473 & 0.899 & 15.662 & 0.993 & 15.138 & 0.853 & 15.015 & 0.567 & 14.737 & 0.532 &  & Bl \\
V160 & 0.65732 & RRab & 15.729 & 1.044 & 15.863 & 1.109 & 15.500 & 0.924 & 15.329 & 0.617 & 15.009 & 0.576 &  & Bl \\
V161 & 0.52515 & RRab & 15.853 & 1.096 & 15.858 & 1.314 & 15.525 & 1.002 & 15.131 & 0.653 & 14.948 & 0.639 &  & Bl \\
V165 & 0.48363 & RRab & 16.014 & 1.260 & 15.790 & 1.503 & 15.452 & 1.325 & 15.516 & 0.747 & 15.139 & 0.720 &  & Bl \\
V166 & 0.32266 & RRd & 16.140 & 0.716 & 15.960 & 0.772 & 15.693 & 0.669 & 15.494 & 0.488 & 15.262 & 0.463 &  & Bl \\
V167 & 0.64396 & RRab & 15.967 & 0.531 & 16.078 & 0.515 & 15.687 & 0.383 & 15.380 & 0.407 & 15.119 & 0.276 & OoI & Bl \\
V168 & 0.27594 & RRc & 15.734 & 0.532 & 15.796 & 0.574 & 15.582 & 0.497 & 15.397 & 0.363 & 15.204 & 0.344 &  & Bl \\
V170 & 0.43230 & RRc & 15.506 & 0.475 & 15.480 & 0.513 & 15.259 & 0.444 & 15.145 & 0.324 & 14.855 & 0.307 &  &  \\
V171 & 0.30506 & RRc & 15.787 & 0.658 & 15.723 & 0.709 & 15.483 & 0.614 & 15.401 & 0.449 & 15.218 & 0.425 &  &  \\
V172 & 0.54229 & RRab & 16.205 & 0.374 & 15.711 & 0.760 & 15.602 & 0.557 & 15.716 & 0.424 & 15.306 & 0.407 &  &  \\
V173 & 0.60700 & RRab & 15.598 & 1.242 & 15.797 & 1.411 & 15.356 & 1.104 & 15.244 & 1.129 & 14.959 & 0.734 &  &  \\
V174 & 0.59130 & RRab & 16.010 & 0.770 & 16.036 & 0.823 & 15.642 & 0.674 & 15.406 & 0.686 & 15.073 & 0.463 &  & Bl \\
V175 & 0.56970 & RRab & 15.988 & 1.169 & 16.075 & 1.146 & 15.714 & 0.815 & 15.406 & 0.689 & 15.163 & 0.558 &  &  \\
V176 & 0.53962 & RRab & 16.065 & 0.794 & 15.989 & 0.846 & 15.693 & 0.692 & 15.536 & 0.706 & 15.222 & 0.469 &  & Bl \\
V177 & 0.34835 & RRc & 15.732 & 0.582 & 15.728 & 0.581 & 15.509 & 0.459 & 15.350 & 0.353 & 15.140 & 0.318 &  &  \\
V178 & 0.26696 & RRc & 15.847 & 0.396 & 15.862 & 0.427 & 15.680 & 0.370 & 15.563 & 0.270 & 15.380 & 0.256 &  &  \\
V180 & 0.60910 & RRab & 15.772 & 0.681 & 16.007 & 0.732 & 15.587 & 0.627 & 15.314 & 0.420 & 15.023 & 0.405 &  &  \\
V181 & 0.66385 & RRab & 15.699 & 0.859 & 15.886 & 0.905 & 15.478 & 0.743 & 15.037 & 0.753 & 14.863 & 0.490 &  &  \\
V184 & 0.53123 & RRab & 15.867 & 1.142 & 15.913 & 1.289 & 15.619 & 1.019 & 15.489 & 0.690 & 15.179 & 0.701 &  & Bl \\
V186 & 0.66325 & RRab & 15.873 & 0.563 & 15.975 & 0.588 & 15.591 & 0.479 & 15.191 & 0.330 & 15.013 & 0.358 &  & Bl \\
V187 & 0.58628 & RRab & 15.951 & 1.199 & 16.030 & 1.065 & 15.643 & 0.761 & 15.411 & 0.658 & 15.152 & 0.539 &  &  \\
V188 & 0.26652 & RRc & 15.880 & 0.429 & 15.902 & 0.463 & 15.693 & 0.401 & 15.604 & 0.293 & 15.392 & 0.278 &  &  \\
V189 & 0.61294 & RRab & 15.782 & 1.012 & 15.946 & 0.901 & 15.503 & 0.737 & 15.311 & 0.601 & 14.919 & 0.409 &  &  \\
V190 & 0.52280 & RRab & 15.947 & 1.356 & 16.013 & 1.396 & 15.673 & 1.082 & 15.277 & 0.892 & 15.196 & 0.688 &  &  \\
V191 & 0.51919 & RRab & 15.815 & 1.356 & 16.033 & 1.457 & 15.678 & 1.266 & 15.615 & 0.742 & 15.257 & 0.654 &  & Bl \\
V192 & 0.49740 & RRab & 14.542 & 0.615 & 14.757 & 0.657 & 14.149 & 0.538 & 13.829 & 0.368 & 13.367 & 0.356 &  & Bl \\
V193 & 0.74787 & RRab & 15.361 & 1.015 & 15.498 & 1.037 & 15.129 & 0.892 & 14.897 & 0.893 & 14.637 & 0.645 &  &  \\
V194 & 0.48920 & RRab & 15.396 & 1.142 & 15.567 & 1.181 & 15.091 & 0.844 & 14.808 & 0.959 & 14.543 & 0.615 &  &  \\
V195 & 0.64392 & RRab & 15.845 & 0.902 & 15.877 & 1.031 & 15.568 & 0.603 & 15.287 & 0.551 & 14.997 & 0.555 &  & Bl \\
V197 & 0.49990 & RRab & 16.113 & 1.238 & 16.086 & 1.443 & 15.718 & 1.175 & 15.194 & 0.719 & 15.275 & 0.717 &  &  \\
V200 & 0.36100 & RRd & 15.393 & 0.821 & 15.820 & 0.885 & 15.500 & 0.913 & 15.256 & 0.560 & 14.985 & 0.531 &  &  \\
V201 & 0.54053 & RRab & 15.186 & 0.948 & 15.571 & 1.079 & 15.142 & 0.882 & 14.836 & 0.574 & 14.828 & 0.577 &  & Bl \\
V202 & 0.77357 & RRab & 15.925 & 0.225 & 15.973 & 0.193 & 15.563 & 0.138 & 15.269 & 0.153 & 14.974 & 0.096 & OoII &  \\
V203 & 0.28980 & RRc & 15.838 & 0.189 & 15.758 & 0.204 & 15.599 & 0.177 & 15.428 & 0.129 & 15.299 & 0.122 &  & Bl \\
V205 & 0.63690 & RRab & 16.035 & 0.648 & 16.128 & 0.483 & 15.716 & 0.421 &  &  & 15.152 & 0.236 & OoI &  \\
V207 & 0.34531 & RRc & 15.698 & 0.609 & 15.816 & 0.657 & 15.526 & 0.569 & 15.264 & 0.433 & 15.079 & 0.394 &  &  \\
V208 & 0.33839 & RRc & 15.769 & 0.429 & 15.801 & 0.476 & 15.511 & 0.401 & 15.254 & 0.293 & 15.026 & 0.278 &  &  \\
V209 & 0.34828 & RRc & 15.818 & 0.520 & 15.799 & 0.561 & 15.556 & 0.486 & 15.373 & 0.427 & 15.181 & 0.336 &  &  \\
V210 & 0.35295 & RRc & 15.883 & 0.581 & 15.919 & 0.627 & 15.668 & 0.543 & 15.438 & 0.460 & 15.243 & 0.376 &  &  \\
V211 & 0.55820 & RRab & 15.908 & 1.182 & 16.125 & 1.106 & 15.721 & 0.943 & 15.256 & 0.605 & 15.295 & 0.624 &  & Bl \\
V212 & 0.54220 & RRab & 15.827 & 1.069 & 15.915 & 1.177 & 15.586 & 0.966 & 15.389 & 0.732 & 15.113 & 0.558 &  & Bl \\
V213 & 0.30000 & RRc & 15.615 & 0.487 & 15.621 & 0.526 & 15.347 & 0.455 & 15.171 & 0.333 & 14.966 & 0.315 &  &  \\
V214 & 0.53951 & RRab & 15.839 & 1.430 & 16.016 & 1.253 & 15.649 & 1.026 & 15.412 & 0.671 & 15.128 & 0.666 &  & Bl \\
V215 & 0.52870 & RRab & 15.594 & 0.914 & 15.708 & 0.991 & 15.412 & 0.812 & 15.244 & 0.533 & 15.085 & 0.536 &  &  \\
V216 & 0.34648 & RRc & 15.745 & 0.533 & 15.828 & 0.575 & 15.560 & 0.498 & 15.380 & 0.363 & 15.161 & 0.344 &  &  \\
V217 & 0.52836 & RRab & 15.476 & 1.406 & 15.728 & 1.194 & 15.387 & 0.982 & 15.264 & 0.942 & 14.948 & 0.679 &  &  \\
V218 & 0.54487 & RRab & 15.920 & 0.982 & 15.992 & 1.020 & 15.630 & 0.843 & 15.414 & 0.510 & 15.067 & 0.562 & OoI & Bl \\
V219 & 0.61361 & RRab & 15.996 & 0.884 & 16.043 & 0.940 & 15.674 & 0.763 & 15.454 & 0.445 & 15.104 & 0.508 &  & Bl \\
V220 & 0.60011 & RRab & 15.954 & 0.658 & 15.988 & 0.899 & 15.606 & 0.793 & 15.354 & 0.698 & 14.966 & 0.424 &  & Bl \\
V221 & 0.37877 & RRc & 15.353 & 0.615 & 15.437 & 0.663 & 15.190 & 0.574 & 15.031 & 0.419 & 14.831 & 0.397 &  &  \\
V222 & 0.59674 & RRab & 15.786 & 0.871 & 15.939 & 1.036 & 15.558 & 0.732 & 15.175 & 0.601 & 15.041 & 0.418 & OoI &  \\
V223 & 0.32923 & RRc & 15.632 & 0.772 & 15.684 & 0.833 & 15.433 & 0.721 & 15.355 & 0.527 & 15.163 & 0.499 &  &  \\
V226 & 0.48843 & RRab & 15.771 & 1.237 & 15.699 & 1.230 & 15.445 & 0.908 & 15.322 & 0.904 & 15.072 & 0.707 &  &  \\
V229 & 0.49762 & RRab & 15.883 & 1.663 & 15.881 & 1.573 & 15.593 & 1.159 & 15.565 & 0.750 & 15.166 & 0.790 &  &  \\
V234 & 0.50802 & RRab & 16.110 & 1.382 & 15.937 & 1.127 & 15.614 & 0.923 & 15.352 & 0.648 & 15.295 & 0.618 &  &  \\
V235 & 0.75984 & RRab & 15.790 & 0.601 & 15.844 & 0.548 & 15.447 & 0.477 & 15.105 & 0.320 & 14.856 & 0.278 & OoII &  \\
V239 & 0.50398 & RRab & 15.930 & 1.022 & 15.971 & 1.292 & 15.654 & 0.915 & 15.523 & 0.940 & 15.203 & 0.763 &  & Bl \\
V240 & 0.27601 & RRc & 15.548 & 0.565 & 15.565 & 0.610 & 15.252 & 0.528 & 14.996 & 0.578 & 14.768 & 0.365 &  &  \\
V241 & 0.59617 & RRab & 15.805 & 1.291 & 15.818 & 1.457 & 15.503 & 1.154 & 15.330 & 0.879 & 15.033 & 0.844 &  &  \\
V242 & 0.59650 & RRab & 15.602 & 0.846 & 15.818 & 0.731 & 15.451 & 0.574 & 15.310 & 0.377 & 14.955 & 0.389 &  &  \\
V243 & 0.63462 & RRab & 15.778 & 0.877 & 15.879 & 0.673 & 15.482 & 0.554 & 15.225 & 0.536 & 14.861 & 0.373 &  & Bl \\
V244 & 0.53784 & RRab & 15.766 & 1.215 & 15.839 & 1.301 & 15.553 & 1.090 & 15.347 & 1.076 & 15.200 & 0.832 &  &  \\
V245 & 0.28403 & RRc & 15.707 & 0.765 & 15.764 & 0.825 & 15.492 & 0.715 & 15.476 & 0.522 & 15.188 & 0.495 &  &  \\
V246 & 0.33914 & RRc & 15.705 & 0.770 & 15.762 & 0.830 & 15.496 & 0.719 & 15.309 & 0.525 & 15.095 & 0.498 &  &  \\
V247 & 0.60536 & RRab & 15.921 & 0.893 & 16.077 & 0.889 & 15.671 & 0.769 & 15.429 & 0.651 & 15.052 & 0.497 &  &  \\
V248 & 0.50979 & RRab & 15.730 & 0.996 & 15.859 & 1.001 & 15.589 & 0.813 & 15.426 & 0.554 & 15.030 & 0.541 &  &  \\
V249 & 0.53300 & RRab & 15.400 & 1.206 & 15.406 & 0.936 & 15.086 & 0.722 & 14.777 & 0.500 & 14.612 & 0.475 &  &  \\
V250n & 0.57438 & RRab & 16.023 & 1.014 & 16.064 & 1.160 & 15.710 & 0.950 & 15.421 & 1.047 & 15.120 & 0.574 &  &  \\
V250s & 0.59242 & RRab & 15.638 & 0.838 & 15.847 & 0.964 & 15.462 & 0.791 & 15.334 & 0.527 & 15.012 & 0.530 &  &  \\
V251 & 0.35392 & RRd & 15.260 & 0.632 & 15.300 & 0.682 & 15.112 & 0.836 & 14.976 & 0.431 & 14.861 & 0.409 &  &  \\
V252 & 0.30350 & RRd & 15.804 & 0.708 & 15.718 & 0.764 & 15.467 & 0.661 & 15.475 & 0.483 & 15.196 & 0.458 &  &  \\
V253 & 0.33262 & RRc & 15.393 & 0.677 & 15.518 & 0.730 & 15.281 & 0.633 & 15.120 & 0.473 & 14.913 & 0.438 &  &  \\
V254 & 0.60564 & RRab & 15.680 & 0.930 & 15.796 & 0.992 & 15.396 & 0.748 & 15.425 & 0.555 & 15.010 & 0.542 &  &  \\
V255 & 0.57271 & RRab & 15.794 & 0.752 & 15.860 & 0.833 & 15.440 & 0.595 & 15.148 & 0.418 & 14.864 & 0.392 &  & Bl \\
V256 & 0.31805 & RRc & 15.894 & 0.937 & 15.857 & 1.011 & 15.644 & 0.876 & 15.456 & 0.639 & 15.295 & 0.606 &  &  \\
V257 & 0.60206 & RRab & 15.698 & 0.818 & 15.768 & 0.886 & 15.425 & 0.705 & 15.300 & 0.751 & 14.916 & 0.426 &  &  \\
V258 & 0.71340 & RRab & 15.896 & 0.632 & 15.971 & 0.649 & 15.584 & 0.500 & 15.334 & 0.439 & 15.001 & 0.321 &  &  \\
V259 & 0.33352 & RRc & 15.481 & 0.399 & 15.501 & 0.431 & 15.080 & 0.373 & 14.815 & 0.272 & 14.467 & 0.258 &  &  \\
V261 & 0.44467 & RRc & 15.146 & 0.988 & 15.188 & 1.065 & 14.875 & 0.923 & 14.631 & 0.674 & 14.538 & 0.639 &  &  \\
V262 & 0.65505 & RRab & 15.664 & 0.527 & 15.880 & 0.569 & 15.479 & 0.467 & 15.439 & 0.294 & 15.015 & 0.261 &  &  \\
V264 & 0.35647 & RRc & 15.700 & 0.879 & 15.647 & 0.948 & 15.287 & 0.821 & 15.228 & 0.600 & 14.946 & 0.568 &  &  \\
V266 & 0.34244 & RRc & 15.630 & 0.562 & 15.710 & 0.606 & 15.411 & 0.525 & 15.234 & 0.575 & 14.967 & 0.358 &  &  \\
V269 & 0.35570 & RRc & 15.212 & 0.625 & 15.329 & 0.674 & 15.062 & 0.553 & 14.988 & 0.640 & 14.807 & 0.404 &  &  \\
V270n & 0.62586 & RRab & 15.740 & 0.653 & 15.814 & 0.799 & 15.457 & 0.659 & 15.254 & 0.563 & 14.930 & 0.386 &  &  \\
V270s & 0.69019 & RRab & 15.041 & 1.059 & 15.088 & 1.195 & 14.873 & 0.861 & 14.558 & 0.624 & 14.514 & 0.620 &  &  \\
V271 & 0.63280 & RRab & 16.084 & 0.817 & 16.088 & 0.807 & 15.674 & 0.594 & 15.403 & 0.340 & 15.069 & 0.367 &  &  \\
V290 & 0.24041 & RRd & 15.881 & 0.115 & 15.851 & 0.124 & 15.674 & 0.107 & 15.547 & 0.078 & 15.374 & 0.074 &  &  \\
V292 & 0.29654 & RRc & 15.785 & 0.472 & 15.778 & 0.509 & 15.603 & 0.441 & 15.501 & 0.322 & 15.331 & 0.305 &  &  \\
% \end{longtable}

% \label{tab:table_1} \textit{Continued on next page}
% \end{table}

